A Probabilistic Calculus of Cyber-Physical Systems

We propose a hybrid probabilistic process calculus for modelling and reasoning on cyber-physical systems (CPSs). The dynamics of the calculus is expressed in terms of a probabilistic labelled transition system in the SOS style of Plotkin. This is used to define a bisimulation-based probabilistic behavioural semantics which supports compositional reasonings. For a more careful comparison between CPSs, we provide two compositional probabilistic metrics to formalise the notion of behavioural distance between systems, also in the case of bounded computations. Finally, we provide a non-trivial case study, taken from an engineering application, and use it to illustrate our definitions and our compositional behavioural theory for CPSs.

==> metricProve.tex <==
%!TEX root=main.tex



\subsection{Proofs of \autoref{sec:metric}}  %\hspace{0.2 cm}
To prove that all $\metric^n$ are 1-bounded pseudometrics (\autoref{prop:up-to-k-metric}), we need some preliminary result.
First we show that the Kantorovich functional $\Kantorovich$ maps pseudometrics to pseudometrics.

\begin{proposition}
\label{prop_kant_metric}
If $d \colon \nome \times \nome \to [0,1]$ is a 1-bounded pseudometric, then also $\Kantorovich(d) \colon \distr{\nome} \times \distr{\nome}$ is a 1-bounded pseudometric.
\end{proposition}
\begin{proof}
To show $\Kantorovich(d)(\gamma,\gamma) = 0$ for all $\gamma \in \distr{\nome}$ it is enough to take the matching $\omega \in \Omega(\gamma,\gamma)$ defined by $\omega(M,M) = \gamma(M)$, for all $M \in \nome$, and $\omega(M,N) = 0$, for all $M,N \in \nome$ with $M \neq N$. 
In fact, we have $\Kantorovich(d)(\gamma,\gamma) \le
\sum_{M,N \in \nome}\omega(M,N) \cdot d(M,N) = \sum_{M \in \nome} \gamma(M) \cdot d(M,M) =0$.

The symmetry $\Kantorovich(d)(\gamma,\gamma') = \Kantorovich(d)(\gamma',\gamma)$ for all $\gamma,\gamma' \in \distr{\nome}$ follows directly by the fact that if we take two functions $\omega,\omega' \colon \nome \times \nome \to [0,1]$ such that $\omega(M,N) = \omega'(N,M)$ for all $M,N \in \nome$, then $\omega \in \Omega(\gamma,\gamma')$ if and only if $\omega' \in \Omega(\gamma',\gamma)$.

To prove the triangle inequality $\Kantorovich(d)(\gamma_1,\gamma_2) \le \Kantorovich(d)(\gamma_1,\gamma_3) + \Kantorovich(d)(\gamma_3,\gamma_2)$ for all $\gamma_1,\gamma_2,\gamma_3 \in \distr{\nome}$, first we consider
the function $\omega \colon \nome \times \nome \to [0,1]$ defined for all $M_1,M_2 \in \nome$ as $\omega(M_1,M_2) = \sum_{M_3 \in \nome \mid \gamma_3(M_3) \neq 0} \frac{\omega_1(M_1,M_3) \cdot \omega_2(M_3,M_2)}{\gamma_3(M_3)}$, where the function $\omega_1 \in \Omega(\gamma_1,\gamma_3)$ is one of the optimal matchings realizing $\Kantorovich(d)(\gamma_1,\gamma_3)$ and $\omega_2 \in \Omega(\gamma_3,\gamma_2)$ one of the optimal matchings realizing $\Kantorovich(d)(\gamma_3,\gamma_2)$.
Then, we prove that
\begin{inparaenum}[(i)]
\item \label{Kant_triang_uno}
$\omega$ is a matching in $\Omega(\gamma_1,\gamma_2)$, and
\item \label{Kant_triang_due}
$\sum_{M_1,M_2 \in \nome} \omega(M_1,M_2) \cdot d(M_1,M_2) \le \Kantorovich(d)(\gamma_1,\gamma_3)  + \Kantorovich(d)(\gamma_3,\gamma_2)$, which immediately implies $\Kantorovich(d)(\gamma_1,\gamma_2) \le \Kantorovich(d)(\gamma_1,\gamma_3)  + \Kantorovich(d)(\gamma_3,\gamma_2)$.
\end{inparaenum}
To show (\ref{Kant_triang_uno}) we prove that the left marginal of $\omega$ is $\gamma_1$ by
\[
\begin{array}{rlr}
& 
\sum_{M_2 \in \nome} \omega(M_1,M_2)
\\
= \quad & \sum_{M_2 \in \nome}  \sum_{M_3 \in \nome \mid \gamma_3(M_3) \neq 0} \frac{\omega_1(M_1,M_3) \cdot \omega_2(M_3,M_2)}{\gamma_3(M_3)}
\\[1.7 ex]
= \quad & \sum_{M_3 \in \nome \mid \gamma_3(M_3) \neq 0} \frac{\omega_1(M_1,M_3) \cdot \gamma_3(M_3)}{\gamma_3(M_3)} & \text{(by $\omega_2 \in \Omega(\gamma_3,\gamma_2)$)}
\\[1.7 ex]
= \quad & \sum_{M_3 \in \nome \mid \gamma_3(M_3) \neq 0} \omega_1(M_1,M_3) 
\\[1.7 ex]
= \quad & \gamma_1(M_1) & \text{(by $\omega_1 \in \Omega(\gamma_1,\gamma_3)$)}
\end{array}
\]
and we observe that the proof that the right marginal of $\omega$ is $\gamma_2$ is analogous.
Then, we show (\ref{Kant_triang_due}) by
\[
\begin{array}{rlr}
&  \sum_{M_1,M_2 \in \nome} \omega(M_1,M_2) \cdot d(M_1,M_2)
\\ 
=  \quad &\sum_{M_1,M_2 \in \nome} \sum_{M_3 \in \nome \mid \gamma_3(M_3) \neq 0} \frac{\omega_1(M_1,M_3) \cdot \omega_2(M_3,M_2)}{\gamma_3(M_3)} \cdot d(M_1,M_2)
\\[1.7 ex]
\le   \quad &  \sum_{M_1,M_2 \in \nome,M_3 \in \nome \mid \gamma_3(M_3) \neq 0} \frac{\omega_1(M_1,M_3) \cdot \omega_2(M_3,M_2)}{\gamma_3(M_3)} \cdot d(M_1,M_3)  \; + 
\\[1.7 ex]
 \quad  &  \sum_{M_1,M_2 \in \nome, M_3 \in \nome \mid \gamma_3(M_3) \neq 0} \frac{\omega_1(M_1,M_3) \cdot \omega_2(M_3,M_2)}{\gamma_3(M_3)} \cdot d(M_3,M_2) 
\\[1.7 ex]
=  \quad &  \sum_{M_1,M_3 \in \nome} \frac{\omega_1(M_1,M_3) \cdot \gamma_3(M_3)}{\gamma_3(M_3)} \cdot  d(M_1,M_3)  +
   \sum_{M_2,M_3 \in \nome} \frac{\gamma_3(M_3) \cdot \omega_2(M_3,M_2)}{\gamma_3(M_3)}  \cdot d(M_3,M_2)
\\[1.7 ex]
=  \quad &  \sum_{M_1,M_3 \in \nome} \omega_1(M_1,M_3) \cdot d(M_1,M_3)  +
   \sum_{M_2,M_3 \in \nome} \omega_2(M_3,M_2)  \cdot d(M_3,M_2)
\\[1.7 ex]
=  \quad &  \Kantorovich(d)(\gamma_1,\gamma_3)  + \Kantorovich(d)(\gamma_3,\gamma_2) 
\end{array}
\]
where the inequality follows from the triangular property of $d$ and the third last equality follows by $\omega_2 \in \Omega(\gamma_3,\gamma_2)$ and $\omega_1 \in \Omega(\gamma_1,\gamma_2)$.
\end{proof}



Now we show that, given any weak bisimulation metric $d$ with $d(M,N) < 1$, then $N$ can mimic weak transitions $M \TransS[\alpha]$ besides those of the form $M \transS[\alpha]$
\begin{lemma} 
\label{lemma_sim_weak_transitions}
Assume a weak bisimulation metric $d$ and $M,N \in \nome$ with $d(M,N) <1$.
If $M \TransS[\hat \alpha] \gamma_M$, then there is a transition $N \TransS[\hat \alpha] \gamma_N$ such that $ \Kantorovich(d)(\gamma_M + (1-\size{\gamma_M}) \dirac{\dummyN}, \gamma_N + (1-\size{\gamma_N}) \dirac{\dummyN}) \le d(M,N)$.
\end{lemma}
\begin{proof}
We proceed by induction on the length $n$ of $s \TransS[\hat \alpha] \gamma_M$.

\underline{Base case $n=1$}. We have two subcases: 
The first is $\alpha = \tau$ and $\gamma_M = \dirac{M}$, the second is $M \transS[\alpha] \gamma_M$.  
In the first case, by definition of $\TransS[\widehat \tau]$ we have $N \TransS[\widehat \tau] \dirac{N}$ and
the thesis holds for $\gamma_N = \dirac{N}$ by observing that $\Kantorovich(d)(\dirac{M} + (1-\size{\dirac{M}})\dirac{\dummyN}),\dirac{N} + (1-\size{\dirac{N}})\dirac{\dummyN}) = \Kantorovich(d)(\dirac{M},\dirac{N}) = d(M,N)$.
In the second case, the thesis follows directly by the definition of weak simulation metric.

\underline{Inductive step $n>1$}.
The derivation $M \TransS[\hat \alpha] \gamma_M$ is obtained by $M \TransS[\hat \beta_1] \rho_M$ and $\rho_M \transS[\hat{\beta}_2] \gamma_M$, for some distribution $\rho_M \in\distr{\nome}$.
The length of the derivation $s \TransS[\hat \beta_1] \rho_M$ is $n-1$ and hence, by the inductive hypothesis, 
there is a transition $t \TransS[\hat \beta_1] \rho_N$ such that $\Kantorovich(d)(\rho_M + (1-\size{\rho_M}) \dirac{\dummyN},\rho_N+ (1-\size{\rho_N}) \dirac{\dummyN}) \le d(M,N)$.
The sub-distributions $\rho_M$ and $\rho_N$ are of the form $\rho_M = \sum_{i \in I}p_i \cdot \dirac{M_i}$ and $\rho_N = \sum_{j \in J}q_j \cdot \dirac{N_j}$.
We have two subcases: The first is $\beta_1=\tau$ and $\beta_2=\alpha$, the other $\beta_1=\alpha$ and $\beta_2=\tau$.

We consider the case $\beta_1=\tau$ and $\beta_2=\alpha$, the other is analogous.
In this case we have $\size{\rho_M} = \size{\rho_N} = 1$ and $\Kantorovich(d)(\rho_M ,\rho_N) \le d(M,N)$.
The transition $\rho_M \transS[\hat{\beta}_2] \gamma_M$ is derived from a $\beta_2$-transition by some of the \CPS{s} $M_i$, namely $I$ is partitioned into sets $I_1 \cup I_2$ such that for all $i \in I_1$ we have $M_i \transS[\beta_2] \gamma_i$ for suitable distributions $\gamma_i$, for each $i \in I_2$ we have $M_i \ntransS[\beta_2]$, and $\rho_M = \sum_{i \in I_1} p_i \gamma_i$.
Analogously, $J$ is partitioned into sets $J_1 \cup J_2$ such that for all $j \in J_1$ we have $N_j \TransS[\hat{\beta_2}] \gamma_j$ for suitable distributions $\gamma_j$ and for each $j \in J_2$ we have $N_j \nTransS[\hat{\beta_2}]$. This gives $\rho_N \TransS[\hat{\beta_2}] \gamma_N$ with $\gamma_N = \sum_{j \in J_1} q_j \cdot \gamma_j$.
Since we had $N \TransS[\hat{\beta_1}] \rho_N$, we can conclude $N \TransS[\hat{\alpha}] \gamma_N$.
In the following we prove that the transitions $N_j \TransS[\hat{\beta_2}] \gamma_j$ can be chosen so that $\Kantorovich(d)(\gamma_M + (1-\size{\gamma_M}) \dummyN,\gamma_N + (1-\size{\gamma_N}) \dummyN) \le d(M,N)$, which concludes the proof.

Let $\omega$ be one of the optimal matchings realizing $\Kantorovich(d)(\rho_M ,\rho_N)$.
We can rewrite the distributions $\rho_M$ and $\rho_N$ as 
$\rho_M = \sum_{i \in I, j \in J} \omega(M_i,N_j) \cdot  \dirac{M_i}$ and 
$\rho_N = \sum_{i \in I, j \in J} \omega(M_i,N_j)  \cdot \dirac{N_j}$.
For all $i \in I_1$ and $j \in J$, define $\gamma_{i,j} = \gamma_i$.
We can rewrite $\gamma_M$ as $\gamma_M = \sum_{i \in I_1,j\in J} \omega(M_i,N_j) \cdot \gamma_{i,j}$.
Analogously, for each $j \in J_1$ and $i \in I$ we note that the transition $q_j \dirac{N_j} \TransS[\hat{\beta_2}] \gamma_{j}$ can always be splitted into $\sum_{i \in I} \omega(M_i,N_j) \cdot \dirac{N_j} \TransS[\hat{\beta_2}] \sum_{i \in I} \omega(M_i,N_j) \cdot \gamma'_{i,j}$
so that we can rewrite $\gamma_j$ as $\gamma_j = \sum_{i \in I}\omega(M_i,N_j)\cdot  \gamma'_{i,j}$ and $\gamma_N$ as
$\gamma_N = \sum_{i\in I, j \in J_1} \omega(M_i,N_j) \cdot \gamma'_{i,j}$. 
Then we note that for all $i \in I_1$ and $j \in J_1$ with $d(M_i,N_j) < 1$, the transition $N_j \TransS[\hat{\beta_2}] \gamma'_{i,j}$ can be chosen so that  
$\Kantorovich(d)(\gamma_{i,j},\gamma'_{i,j} + (1-\size{\gamma'_{i,j}})\dummyN) \le d(M_i,N_j)$.

For all $i \in I_1$ and $j \in J_1$ with $d(M_i,N_j) <1$, let $\omega_{i,j}$ be one of the optimal matchings realizing $\Kantorovich(d)(\gamma_{i,j}, \gamma_j + (1-\size{\gamma_j}) \dummyN)$.
Define $\omega' \colon \nome \times \nome \to [0,1]$ as the function such that 
\[ 
\omega'(M',N') = 
\begin{cases} 
\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(M',N') 
& \text{ if } M' \neq \dummyN \neq N'\\
\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(M',N') + \sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(M')
& \text{ if } M' \neq \dummyN = N' \\
\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(M',N') + \sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(N')
& \text{ if } M' = \dummyN \neq N' \\
\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(M',N') +  \sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(M') + \\
 \sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(N')+ \sum_{i \in I_2, j \in J_2}\omega(M_i,N_j) 
& \text{ if } M' = \dummyN = N'. 
\end{cases}
\] 

To infer the proof obligation $\Kantorovich(d)(\gamma_M + (1-\size{\gamma_M}) \dirac{\dummyN},\gamma_N + (1-\size{\gamma_N}) \dirac{\dummyN}) \le d(M,N)$ we show that
\begin{inparaenum}[(i)]
\item \label{matching} $\omega'$ is a matching in $\Omega(\gamma_M + (1-\size{\gamma_M}) \dirac{\dummyN},\gamma_N + (1-\size{\gamma_N}) \dirac{\dummyN})$, and
\item \label{metric_condition} $\sum_{M',N' \in \nome} \omega'(M',N') \cdot d(M',N') \le d(M,N)$.
\end{inparaenum}

To show (\ref{matching}) we prove that the left marginal of $\omega'$ is $\gamma_M + (1-\size{\gamma_M}) \dirac{\dummyN}$.
The proof that the right marginal is $\gamma_N + (1-\size{\gamma_N}) \dirac{\dummyN})$ is analogous.
For any \CPS{} $M' \neq \dummyN$, we have
$\sum_{N' \in \nome}\omega'(M',N')$ = 
$\sum_{N' \neq \dummyN} \sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(M',N')$ 
+
$\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(M',\dummyN)$ 
+ 
$\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(M')$ 
=
$\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \sum_{N' \in \nome} \omega_{i,j}(M',N')$ 
+ 
$\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(M')$ 
= (since $\omega_{i,j}$ is a matching in $\Omega(\gamma_{i,j},\gamma'_{i,j})$)
$\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \gamma_{i,j}(M')$ 
+ 
$\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(M')$ 
=
$\sum_{i \in I_1, j \in J}\omega(M_i,N_j) \cdot \gamma_{i,j}(M')$ 
= $(\gamma_M+ (1-\size{\gamma_M}) \dummyN)(M')$. 

%Consider now the \CPS{} 
Consider now the \CPS{} $\dummyN$. In this case we have that
$\sum_{N' \in \nome}\omega'(\dummyN,N')$ equals the summation
$\sum_{N' \neq \dummyN}\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(\dummyN,N')$ 
+ $\sum_{N' \neq \dummyN} \sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(N')$ 
+ $\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(\dummyN,\dummyN)$ 
+  $\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(\dummyN)$ 
+ $\sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(\dummyN)$
+ $\sum_{i \in I_2, j \in J_2}\omega(M_i,N_j)$.
Then, this summation is equal to 
$\sum_{N' \in \nome}\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(\dummyN,N')$ +
$\sum_{N' \in \nome} \sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(N')$ +
$\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(\dummyN)$ +
$\sum_{i \in I_2, j \in J_2}\omega(M_i,N_j)$. 
Since $\omega_{i,j}$ is a matching in $\Omega(\gamma_{i,j},\gamma'_{i,j})$, the first summand is
$\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \gamma_{i,j}(\dummyN)$.
Then, since $\gamma'_{i,j}$ is a distribution, the second summand is 
$\sum_{i \in I_2, j \in J_1}\omega(M_i,N_j)$.
Overall we obtain
$\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \gamma_{i,j}(\dummyN)$ +
$\sum_{i \in I_2, j \in J_1}\omega(M_i,N_j)$ +
$\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(\dummyN)$ +
$\sum_{i \in I_2, j \in J_2}\omega(M_i,N_j)$ 
= 
$\sum_{i \in I_1, j \in J}\omega(M_i,N_j) \cdot \gamma_{i,j}(\dummyN)$ +
$\sum_{i \in I_2, j \in J}\omega(M_i,N_j)$
=
$(\gamma_M + (1-\size{\gamma_M}) \dirac{\dummyN})(\dummyN)$, 
where in the last step we exploit $\sum_{i \in I_1, j \in J}\omega(M_i,N_j) = \sum_{i \in I_1} p_i = \size{\gamma_M}$.

To prove (\ref{metric_condition}), by looking at the definition of $\omega'$ above we get that $\sum_{M',N' \in \nome} \omega'(M',N') \cdot d(M',N')$ is the summation of the following values:
\begin{itemize}
\item
$\sum_{M' \neq \dummyN \neq N'} \sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(M',N') \cdot d(M',N')$
\item
$\sum_{ M' \neq \dummyN}\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(M',\dummyN) \cdot d(M',\dummyN) + \sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(M') \cdot d(M',\dummyN)$
\item
$\sum_{N' \neq \dummyN}\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot  \omega_{i,j}(\dummyN,N') \cdot d(\dummyN,N') + \sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(N') \cdot d(\dummyN,N')$
\item
$\sum_{i \in I_1, j \in J_1}\omega(M_i,N_j) \cdot \omega_{i,j}(\dummyN,\dummyN) \cdot d(\dummyN,\dummyN)+  \sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(\dummyN) \cdot d(\dummyN,\dummyN)
+ \sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(\dummyN)\cdot d(\dummyN,\dummyN)+ \sum_{i \in I_2, j \in J_2}\omega(M_i,N_j)\cdot d(\dummyN,\dummyN)$.
\end{itemize}
By moving the first summand of the second, third and fourth items to the first item, we rewrite this summation as the summation of the following values:
\begin{itemize}
\item
$\sum_{M' , N' \in \nome} \sum_{i \in I_1, j \in J_1} \omega(M_i,N_j) \cdot \omega_{i,j}(M',N') \cdot d(M',N')$
\item
$\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(M') \cdot d(M',\dummyN)$
\item
$\sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(N') \cdot d(\dummyN,N')$
\item
$\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \cdot \gamma_{i,j}(\dummyN) \cdot d(\dummyN,\dummyN)
+ \sum_{i \in I_2, j \in J_1}\omega(M_i,N_j) \cdot \gamma'_{i,j}(N')\cdot d(\dummyN,\dummyN)+ \sum_{i \in I_2, j \in J_2}\omega(M_i,N_j)\cdot d(\dummyN,\dummyN)$.
\end{itemize}
By the definition of $\omega_{i,j}$ the first item is $\sum_{i \in I_1, j \in J_1} \omega(M_i,N_j) \Kantorovich(d)(\gamma_{i,j},\gamma'_{i,j})$.
If $d(M_i,N_j) < 1$, we chosen $\gamma'_{i,j}$ such that $\Kantorovich(d)(\gamma_{i,j},\gamma'_{i,j}) \le d(M_i,N_j)$.
If $d(M_i,N_j) = 1$, then $\Kantorovich(d)(\gamma_{i,j},\gamma'_{i,j}) \le d(M_i,N_j)$ is immediate.
Henceforth we are sure that in all cases the first item is less or equal $\sum_{i \in I_1, j \in J_1} \omega(M_i,N_j) \cdot d(M_i,N_j)$.
The second item is clearly less or equal than $\sum_{i \in I_1, j \in J_2}\omega(M_i,N_j)$.
The third item is 0, since $d(\dummyN,N') = 0$ for all $N' \in \nome$.
Finally, the last item is 0 since $d(\dummyN,\dummyN) = 0$.
Namely, $\sum_{M',N' \in \nome} \omega'(M',N') \cdot d(M',N') \le \sum_{i \in I_1, j \in J_1} \omega(M_i,N_j) \cdot d(M_i,N_j) + \sum_{i \in I_1, j \in J_2}\omega(M_i,N_j)$.
Since $\Kantorovich(d)(\rho_M ,\rho_N )$ is the summation of the following values:
\begin{itemize}
\item
$\sum_{i \in I_1,j\in J_1} \omega(M_i,N_j) \cdot d(M_i,N_j)$
\item
$\sum_{i \in I_1,j\in J_2} \omega(M_i,N_j) \cdot d(M_i,N_j) = \sum_{i \in I_1,j\in J_2} \omega(M_i,N_j)$ ($M_i \trans{\beta_2}$ and $N_j \not\!\!\TransS[\hat{\beta_2}]$ give $d(M_i,N_j) =1$) 
\item
$\sum_{i \in I_2,j\in J_1} \omega(M_i,N_j) \cdot d(M_i,N_j)$ 
\item
$\sum_{i \in I_2,j\in J_2} \omega(M_i,N_j) \cdot d(M_i,N_j)$.
\end{itemize}
it is immediate that $\sum_{i \in I_1, j \in J_1} \omega(M_i,N_j) \cdot d(M_i,N_j) + \sum_{i \in I_1, j \in J_2}\omega(M_i,N_j) \le \Kantorovich(d)(\rho_M ,\rho_N )$.
Since we had $\Kantorovich(d)(\rho_M ,\rho_N) \le d(M,N)$ we can conclude $\sum_{M',N' \in \nome} \omega'(M',N') \cdot d(M',N') \le d(M,N)$, as required.
\end{proof}

We are now ready to prove that all $\metric^n$ are pseudometrics.
\\

\noindent
\textbf{Proof of  \autoref{prop:up-to-k-metric}} \hspace{0.2 cm}
We have to prove that $\metric^{n}(M,M) = 0$,  $\metric^{n}(M,N) = \metric^n(N,M)$ and $\metric^{n}(M,N) \le \metric^{n}(M,O)+\metric^{n}(O,N)$ for all $M,N,O \in \nome$.
We reason by induction over $n$. 
The base case $n=0$ is immediate since $\metric^0(M,N) = 0$ for all $M,N \in \nome$.
We consider the inductive step $n+1$.

%%% vecchio case base k=1 rimosso
\begin{comment}
\underline{Base case $n=1$}.

Let us start with proving $\metric^{1}(M,M) = 0$.
We have to show that for each transition $M \transS[\alpha] \gamma$ there is a transition $M \TransS[\hat{\alpha}] \rho$ with 
$ \Kantorovich(\zeroF)(\gamma, \rho+ (1-\size{\rho})\dirac{\dummyN}) = 0$.
We choose $\rho = \gamma$ and the transition $M \transS[\alpha] \gamma$.
We obtain $ \Kantorovich(\zeroF)(\gamma, \rho + (1-\size{\rho})\dirac{\dummyN})$ = $\Kantorovich(\zeroF)(\gamma,\gamma)$ = $0$, where the last equality follows by the definition of $\zeroF$.

Then we prove the symmetry $\metric^{1}(M,N) = \metric^1(N,M)$. We have
\[\begin{array}{rl}
& 
\metric^{1}(M,N) \\
%
= &
\Bisimulation(\zeroF)(M,N) \\
%
= & 
\displaystyle \max_{\alpha \in \ActComp} \max\left\{ \max_{M \transS[\alpha]\gamma_1} \min_{N \TransS[\alpha]\in \gamma_2} \Kantorovich(\zeroF)(\gamma_1,\gamma_2 + (1-\size{\gamma_2})\dirac{0}), 
\max_{N \transS[\alpha] \gamma_2}\min_{M \TransS[\alpha]\gamma_1} \Kantorovich(\zeroF)(\gamma_1+ (1-\size{\gamma_1})\dirac{0},\gamma_2)  \right\} \\
%
= & 
\displaystyle \max_{\alpha \in \ActComp} \max\left\{ \max_{M \TransS[\alpha]\gamma_1} \min_{N \TransS[\alpha]\in \gamma_2} \Kantorovich(\zeroF)(\gamma_1,\gamma_2 + (1-\size{\gamma_2})\dirac{0}), 
\max_{N \TransS[\alpha] \gamma_2}\min_{M \TransS[\alpha]\gamma_1} \Kantorovich(\zeroF)(\gamma_1+ (1-\size{\gamma_1})\dirac{0},\gamma_2)  \right\} \\
%
= & 
\Bisimulation(\zeroF)(N,M) \\
%
= & 
\metric^1(N,M)
\end{array}
\]
where the third equality follows by \autoref{lemma_sim_weak_transitions}.


Finally we prove the triangular property $\metric^{1}(M,N) \le \metric^{1}(M,O) +\metric^{1}(O,N)$.
It is immediate if $\metric^{1}(M,O) =1$ or $\metric^{1}(O,N) =1$.
Otherwise, it is enough to prove that any transition $M \transS[\alpha] \gamma_M$ is mimicked by a transition $N \TransS[\hat{\alpha}] \gamma_N$ with $ \Kantorovich(\zeroF)(\gamma_M,\gamma_N + (1-\size{\gamma_N})\dummyN) \le \metric^{1}(M,N) + \metric^{1}(M,N)$.
From $M \transS[\alpha] \gamma_M$ and $\metric^{1}(M,O) < 1$ there is a transition $O \TransS[\hat{\alpha}] \gamma_O$,
and, 
by  \autoref{lemma_sim_weak_transitions}, from $O \TransS[\hat{\alpha}] \gamma_O$ and $\metric^{1}(O,N) <1$ there is a transition $t \TransS[\hat{\alpha}] \gamma_N$.
By definition of $\zeroF$ we have $ \Kantorovich(\zeroF)(\gamma_M,\gamma_N + (1-\size{\gamma_N})\dummyN) = 0$, which is trivially less or equal than $\metric^{1}(M,O) + \metric^{1}(O,N)$. 

\end{comment}
%% vecchio caso base k=1 rimosso

%\underline{Inductive step $n+1$}.

Let us start with proving $\metric^{n+1}(M,M) = 0$.
We have to show that for each transition $M \transS[\alpha] \gamma$ there is a transition $M \TransS[\hat{\alpha}] \rho$ with 
$ \Kantorovich(\metric^{n})(\gamma, \rho + (1-\size{\rho})\dirac{\dummyN}) = 0$.
We choose $\rho = \gamma$ and the transition $M \transS[\alpha] \gamma$.
We obtain $ \Kantorovich(\metric^{n})(\gamma, \rho + (1-\size{\rho})\dirac{\dummyN})$ = $ \Kantorovich(\metric^{n})(\gamma,\gamma)$ = $0$, with the last equality by the inductive hypothesis and  \autoref{prop_kant_metric}. 

%Then we prove the symmetry 
The symmetry $\metric^{n+1}(M,N) = \metric^{n+1}(N,M)$ follows by 
$ \metric^{n+1}(M,N) = \Bisimulation(\metric^{n})(M,N) = \Bisimulation(\metric^{n})(N,M) = \metric^{n+1}(N,M)$, where the second equality follows immediately by the definition of $\Bisimulation$.
\begin{comment}
Define $A= \{\alpha : M \transS[\alpha] \vee N \transS[\alpha]\}$.
\remarkR{c'e' una d di troppo e nelle formule qui sotto, nella terza e quarta c'e' un appartiene di troppo}
\remarkS{non vedo gli appartiene!}
We have
\[\begin{array}{rl}
& 
\metric^{n+1}(M,N) \\
= &
\Bisimulation(\metric^{n})(M,N) \\
= & 
\displaystyle \max_{\alpha \in A} \max \Big\{ \max_{M \transS[\alpha]\gamma_1} \min_{N \TransS[\alpha]\in \gamma_2} \Kantorovich(\metric^{n})(\gamma_1,\gamma_2 + (1-\size{\gamma_2})\dirac{\dummyN}), 
\max_{N \transS[\alpha] \gamma_2}\min_{M \TransS[\alpha]\gamma_1} \Kantorovich(\metric^{n})(\gamma_1+ (1-\size{\gamma_1})\dirac{\dummyN},\gamma_2)  \Big\} \\
= & 
\displaystyle \max_{\alpha \in A} \max \Big\{ \max_{M \TransS[\alpha]\gamma_1} \min_{N \TransS[\alpha]\in \gamma_2} \Kantorovich(\metric^{n})(\gamma_1,\gamma_2 + (1-\size{\gamma_2})\dirac{\dummyN}), 
\max_{N \TransS[\alpha] \gamma_2}\min_{M \TransS[\alpha]\gamma_1} \Kantorovich(\metric^{n})(\gamma_1+ (1-\size{\gamma_1})\dirac{\dummyN},\gamma_2)  \Big\} \\
= & 
\displaystyle \max_{\alpha \in A} \max \Big\{ \max_{N \TransS[\alpha] \gamma_2}\min_{M \TransS[\alpha]\gamma_1} \Kantorovich(\metric^{n})(\gamma_1+ (1-\size{\gamma_1})\dirac{\dummyN},\gamma_2)  ,
 \max_{M \TransS[\alpha]\gamma_1} \min_{N \TransS[\alpha]\in \gamma_2} \Kantorovich(\metric^{n})(\gamma_1,\gamma_2 + (1-\size{\gamma_2})\dirac{\dummyN}) \Big\} \\
= & 
\displaystyle \max_{\alpha \in A} \max \Big\{ \max_{N \transS[\alpha] \gamma_2}\min_{M \TransS[\alpha]\gamma_1} \Kantorovich(\metric^{n})(\gamma_1+ (1-\size{\gamma_1})\dirac{\dummyN},\gamma_2)  ,
 \max_{M \transS[\alpha]\gamma_1} \min_{N \TransS[\alpha]\in \gamma_2} \Kantorovich(\metric^{n})(\gamma_1,\gamma_2 + (1-\size{\gamma_2})\dirac{\dummyN}) \Big\} \\
= & 
\Bisimulation(\metric^{n})(N,M) \\
= & 
\metric^{n+1}(N,M) \enspace .
\end{array}
\]
where the third and fifth equalities follows by \autoref{lemma_sim_weak_transitions}.
\remarkR{sicuro che usi il lemma 2 ?}
\remarkS{si}
\end{comment}


Finally we prove the triangular property $\metric^{n+1}(M,N) \le \metric^{n+1}(M,O) +\metric^{n+1}(O,N)$.
This result is immediate if $\metric^{n+1}(M,O) =1$ or $\metric^{n+1}(O,N) =1$.
Otherwise, it is enough to prove that any $M \transS[\alpha] \gamma_M$ is mimicked by some transition $N \TransS[\hat{\alpha}] \gamma_N$ with $ \Kantorovich(\metric^{n})(\gamma_M,\gamma_N + (1-\size{\gamma_N})\dirac{\dummyN}) \le \metric^{n+1}(M,O) + \metric^{n+1}(O,N)$.
From $M \transS[\alpha] \gamma_M$ and $\metric^{n+1}(M,O) < 1$ we immediately infer that there is a transition $O \TransS[\hat{\alpha}] \gamma_O$ with $ \Kantorovich(\metric^{n})(\gamma_M ,\gamma_O + (1-\size{\gamma_O})\dirac{\dummyN}) \le \metric^{n+1}(M,O)$.
By  \autoref{lemma_sim_weak_transitions}, from $O \TransS[\hat{\alpha}] \gamma_O$ and $\metric^{n+1}(O,N) <1$ there is a transition $N \TransS[\hat{\alpha}] \gamma_N$ such that $ \Kantorovich(\metric^{n})(\gamma_O + (1-\size{\gamma_O})\dirac{\dummyN},\gamma_N + (1-\size{\gamma_N})\dirac{\dummyN}) \le \metric^{n+1}(O,N)$.
By the inductive hypothesis and  \autoref{prop_kant_metric} we get that  $\Kantorovich(\metric^{n})$ is a pseudometric, hence it satisfies the triangle inequality, namely $\Kantorovich(\metric^{n})(\gamma_M,\gamma_N+ (1-\size{\gamma_N})\dirac{\dummyN}) \le \Kantorovich(\metric^{n})(\gamma_M, \gamma_O + (1-\size{\gamma_O})\dirac{\dummyN}) + \Kantorovich(\metric^{n})(\gamma_O+ (1-\size{\gamma_O}) \dirac{\dummyN},\gamma_N + (1-\size{\gamma_N})\dirac{\dummyN})$.
Therefore we can conclude the proof by $\Kantorovich(\metric^{n})(\gamma_M,\gamma_N+ (1-\size{\gamma_N})\dirac{\dummyN}) \le  \Kantorovich(\metric^{n})(\gamma_M, \gamma_O + (1-\size{\gamma_O})\dirac{\dummyN}) +  \Kantorovich(\metric^{n})(\gamma_O+ (1-\size{\gamma_O}) \dirac{\dummyN},\gamma_N + (1-\size{\gamma_N})\dirac{\dummyN})
 \le \metric^{n+1}(M,O) + \metric^{n+1}(O,N)$.
\qed
\\







\noindent
\textbf{Proof of  \autoref{prop:metric_as_a_limit}} \hspace{0.2 cm}
Follows by the same arguments in \cite{vB12}.
\qed
\\


\begin{comment}


\begin{proof}[Proof of  \autoref{prop:metric_is_a_metric}]
First we show that $\metric$ is a 1-bounded pseudometric.
We have to prove 
\begin{inparaenum}[(i)] 
\item
$\metric(M,M) = 0$, 
\item
$\metric(M,N) = \metric(N,M)$, and 
\item
$\metric(M,N) \le \metric(M,O)+\metric(O,N)$.
\end{inparaenum}
By applying  \autoref{prop:metric_as_a_limit} and  \autoref{prop:up-to-k-metric} we obtain
\begin{inparaenum}[(i)]
\item
$\metric(M,M)  = \lim_{k \to \infty}\metric^n(M,M) = \lim_{k \to \infty}0 = 0$,
\item
$\metric(M,N)  = \lim_{k \to \infty}\metric^n(M,N) = \lim_{k \to \infty}\metric^n(N,M) =\metric(N,M)$, and
\item
$\metric(M,N) = \lim_{k \to \infty}\metric^n(M,N) \le \lim_{k \to \infty}( \metric^n(M,O)+\metric^n(O,N)) \le \lim_{k \to \infty} \metric^n(M,O) + \lim_{k \to \infty} \metric^n(O,N) =  \metric(M,O)+\metric(O,N)$.
\end{inparaenum}
Then, since $\metric$ is a 1-bounded pseudometric and is a prefixed point of $\Bisimulation$, we infer that it is a simulation metric.
Since all simulation metrics are prefixed points of $\Bisimulation$, $\metric$ is the minimal one.
\end{proof}
\end{comment}




In order to prove the compositionality or our weak bisimilarity metrics, i.e.\ \autoref{thm:congruenceP}, we divide its statement in six different propositions.
To prove that $\approx_p$ preserves contextuality, we need a number of technical lemmas. 
\autoref{lem:aux2P} formalises a number of properties of the compound environment $E_1\uplus E_2$. 
\begin{lemma}
\label{lem:aux2P}
Let $E_1$ and $E_2$ be two physical environments. 
If defined, the environment $E_1 \uplus E_2$ has the following properties:
\begin{enumerate} 
\item 
\label{uno}
$\mathit{read\_sensor}(E_1\uplus E_2,s)  $ is equal to $\mathit{read\_sensor}(E_1 ,s)$, if $s$ is a sensor  of $E_1$, and it is equal to $\mathit{read\_sensor}(E_2 ,s)$, if $s$ is a sensor  of $E_2$;
%
\item 
\label{unobisP}
For a distribution $D$ over reals, $D \in \mathit{read\_sensor}(E_1 ,s)$ implies $D \in \mathit{read\_sensor}(E_1\uplus E_2,s)$, for any sensor $s$ in $E_1$ and for any environment $E_2$;
%
\item 
\label{due}
$\mathit{update\_act}(E_1\uplus E_2,a,v)  $  is equal to $\mathit{update\_act}(E_1 ,a,v)  \uplus E_2$, if $a$ is an actuator of $E_1$, and it is equal to $E_1 \uplus \mathit{update\_act}(  E_2,a,v)$, if $a$ is an actuator of $E_2$;
%
\item 
\label{duebis}
$\mathit{update\_act}(E_1 ,a,v)  \uplus E_2$  is equal to $\mathit{update\_act}(E_1\uplus E_2,a,v)  $   for any actuator $a$ in $E_1$ and for any environment $E_2$;
%
\item 
\label{treP}
$(\mathit{next}(E_1\uplus E_2))(E_1'\uplus E_2'  ) =(\mathit{next}(E_1))(E_1') \cdot (\mathit{next}(E_2))(E_2')$;
%
\item 
\label{quattro}
$\invariantfun{}(E_1\uplus E_2) =\invariantfun{}(E_1 ) \wedge \invariantfun{}( E_2)$.
\end{enumerate}
\end{lemma}
\begin{proof}
By definition of the operator $\uplus$ on physical environments.
\end{proof}



%\remarkR{prove da aggiustare causa Dead}


Given a distribution $\gamma$ over \CPS{s} and a \CPS{} $O$, we denote with $\gamma \uplus O$ the distribution defined by $(\gamma \uplus O)(M \uplus O) = \gamma(M)$ for all \CPS{s} $M$.
\autoref{lem:aux1P} serves to propagate untimed actions on parallel \CPS{s}. 

\begin{lemma}
\label{lem:aux1P}
If $M  \trans{\alpha} \gamma$, with $\alpha \neq \tick$,
then $M \uplus O \trans{\alpha} \gamma \uplus O$, for any non-interfering \CPS{} $O$, with $\invariantfun{}(O)=\true$. 
\end{lemma}

\begin{proof}
If $M$ is the \CPS{} $\dummyN$ then also $M \uplus O$ is $\dummyN$  and the thesis is immediate. 
Consider the case $M \neq \dummyN$.
Let us assume that $M=\confCPS {E_1}  {P_1}$ and  $O=\confCPS {E_2}  {P_2}$, for some environments $E_1$ and $E_2$ and processes $P_1$ and $P_2$. 
We consider the case in which $M \trans{\alpha} \gamma$ is derived by rule \rulename{SensRead}.
The other cases where the transition is derived by the other rules in \autoref{tab:lts_systems_P} can be proved in a similar manner.
In this case, we have $\alpha=\tau$ and there are a sensor $s$, probability values $p_i$ and real values $v_i$ with $i\in I$ and a process $P'_1$ such that 
the rule \rulename{SensRead} instances as 
\[
\Txiombis
{P_1  \trans{\rcva s z} P_1'  \Q \Q \invariantfun{}(E_1 ) \Q \Q 
\mbox{\small{$\mathit{read\_sensor}(E_1 ,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$}} 
}
{M   \trans{\tau} \gamma }
\]
with $\gamma=\confCPS {\overline{E_1}} {\sum_{i \in I}p_i \cdot \dirac{P'_1\subst{v_i}{z}}}$.

Now we argue that we can apply rule \rulename{SensRead} to infer a transition by $M \uplus O$. 
Recall that $M \uplus O$ is the \CPS{} $\confCPS {E_1 \uplus E_2}{P_1 \parallel P_2}$.
From $P_1  \trans{\rcva s z} P'_1$, by rule \rulename{Par} in \autoref{tab:lts_processes} we can derive the transition
$P_1 \parallel P_2 \trans{\rcva s z} P'_1 \parallel P_2$, which is one of the premises of  rule \rulename{SensRead} necessary to infer a transition by $\confCPS {E_1 \uplus E_2}{P_1 \parallel P_2}$.
Then, the premise $\invariantfun{}(E_1 \uplus E_2 )$ of  \rulename{SensRead} follows by the validity of $\invariantfun{}(E_1 )$, the hypothesis $\invariantfun{}(E_2 )=\true$ and \autoref{lem:aux2P}(\ref{quattro}).
Finally, the premise $\mathit{read\_sensor}(E_1\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$ follows by
$\mathit{read\_sensor}(E_1 ,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$ and \autoref{lem:aux2P}(\ref{unobisP}).
Therefore we have
\[
\Txiombis
{P_1 \parallel P_2 \trans{\rcva s z} P'_1 \parallel P_2 \Q\Q \invariantfun{}(E_1\uplus E_2) \Q\Q
\mbox{\small{$\mathit{read\_sensor}(E_1\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$}} 
}
{M \uplus O \trans{\tau}\confCPS {\dirac{E_1\uplus E_2}} {\sum_{i \in I}p_i \cdot \dirac{(P'_1 \parallel P_2)\subst{v_i}{z}}}} \enspace 
\]
with  $\confCPS {\dirac{E_1\uplus E_2}} {\sum_{i \in I}p_i \cdot \dirac{(P'_1 \parallel P_2})\subst{v_i}{z}}  = 
(\confCPS {\overline{E_1}} {\sum_{i \in I}p_i \cdot \dirac{P'_1\subst{v_i}{z}}}) \uplus (\confCPS {\dirac{E_2}}{P_2}) = \gamma \uplus O$.
\end{proof}

\autoref{lem:aux1P} can be generalized to weak transitions.

\begin{lemma}
\label{lem:aux1Pbis}


If $M  \TransS[\widehat{\alpha}] \gamma$, with $\alpha \neq \tick$,
then $M \uplus O  \TransS[\widehat{\alpha}]  \gamma \uplus O$, for any non-interfering \CPS{} $O$, with $\invariantfun{}(O)=\true$. 
\end{lemma}
\begin{proof}
By induction over the length $n$ of $\TransS[\widehat{\alpha}]$.
The base case $n=1$ is given by \autoref{lem:aux1P}.
Consider the inductive step $n+1$.
We have $M \TransS[\widehat{\alpha_1}] \gamma' \transS[\widehat{\alpha_2}] \gamma$ with either $\alpha_1 = \alpha$ and $\alpha_2 = \tau$, or $\alpha_1 = \tau$ and $\alpha_2 = \alpha$.
%We consider the case $\alpha_1 = \alpha$ and $\alpha_2 = \tau$, the other is similar.
Since the length of $\TransS[\widehat{\alpha_1}]$ is $n$, we can apply the inductive hypothesis and infer 
$M \uplus O  \TransS[\widehat{\alpha_1}]  \gamma' \uplus O$.
Assume $\gamma' = \sum_{i \in I}p_i \cdot \dirac{M_i}$, for suitable probability values $p_i$ and \CPS{} $M_i$. 
By definition, $\gamma' \transS[\widehat{\alpha_2}] \gamma$ implies that there exists a subset $J \subseteq I$ with
$M_j \transS[\widehat{\alpha_2}] \gamma_j$ for all $j \in J$, $M_i \ntransS[\alpha_2]$ for $i \in I \setminus J$ and $\gamma = \sum_{j \in J} p_j \cdot \dirac{M_j}$.
We can prove now that for any $j \in J$ we have $M_j \uplus O \transS[\widehat{\alpha_2}] \gamma_j\ \uplus O$.
We distinguish two cases.
The first case is $M_j \transS[\alpha_2] \gamma_j$. 
By \autoref{lem:aux1P} we get $M_j \uplus O \transS[\alpha_2] \gamma_j\ \uplus O$, and, therefore, $M_j \uplus O \transS[\widehat{\alpha_2}] \gamma_j\ \uplus O$.
The second case is $\alpha_2 = \tau$ and $\gamma_j = \dirac{M_j}$.
We immediately have $M_j \uplus O \transS[\widehat{\tau}] \gamma_j\ \uplus O$.
Hence $\sum_{j\in J} M_j \uplus O \transS[\widehat{\alpha_2}] \sum_{j \in J} \gamma_j  \uplus O$, namely  $\gamma' \uplus O \transS[\widehat{\alpha_2}] \gamma \uplus O$.
Then, from $M \uplus O  \TransS[\widehat{\alpha_1}]  \gamma' \uplus O$ and $\gamma' \uplus O \transS[\widehat{\alpha_2}] \gamma \uplus O$ we get $M \uplus O  \TransS[\widehat{\alpha}] \gamma \uplus O$, which completes the proof.
\end{proof}


Next lemma says that the invariants of \CPS{s} in distance $< 1$ must agree.

\begin{lemma}
\label{lem:bis-invP}
$\metric(M , N) < 1$ for $M,N \neq \dummyN$ implies $\invariantfun{}(M) = \invariantfun{}(N)$.
\end{lemma}
\begin{proof}

The proof is by contradiction. 
Assume that $\metric(M , N) < 1$, $\invariantfun{}(M) = \true$ and $ \invariantfun{}(N)=\false$.
We show that $M \TransS[\widehat{\tick}]$ and $N \nTransS[\widehat{\tick}]$, which contradicts $\metric(M , N) < 1$.
By well timedness property for \CPS{s} (\autoref{prop:time}), there exists a natural $n$ such that all derivations $M  \trans{\tau} M_1 \trans{\tau}\dots \trans{\tau} M_k$ are such that $k \le n$, then we have $M_k \ntrans \tau$. 
Since $M_n \ntrans \tau$, by the maximal progress property for \CPS{s} (\autoref{prop:time}) it follows that $M_n \trans \tick \gamma$, for some $\gamma$.
We conclude $M \TransS[\widehat{\tick}]$. 
Since $ \invariantfun{}(N)=\false$, the \CPS{} $N$ can  perform only the step  $N\trans \tau \dummyN$ and $\dummyN$ can not perform  any 
action, and hence, $N \nTransS[\widehat{\tick}]$. 
\end{proof}

Here comes one of the main technical result: the bisimilarity metric is preserved by the parallel composition of non-interfering \CPS{s}. 
\begin{proposition}
\label{lem:cong1P}
$\metric(M \uplus O ,N \uplus O) \le \metric(M , N) $, for any physically disjoint \CPS{} $O$. 
\end{proposition}
\begin{proof}
The case $\metric(M , N) = 1$ is immediate, therefore we assume $\metric(M , N) < 1$. 
Let us define the function $d \colon \nome \times \nome \to [0,1]$ by $d(M \uplus O , N \uplus O) = \metric(M,N)$ for all $M,N,O \in \nome$.
To prove the thesis it is enough to show that $d$ is a weak bisimulation metric. 
In fact, since $\metric$ is the minimal weak bisimulation metric, we infer $\metric \sqsubseteq d$, thus giving $\metric(M \uplus O , N \uplus O) \le d(M \uplus O , N \uplus O) = \metric(M,N)$.
To prove that $d$ is a weak bisimulation metric, we show that any transition $M \uplus  O \trans{\alpha} \gamma$ is simulated by some transition $N \uplus  O \TransS[\widehat{\alpha}] \gamma'$ with $\Kantorovich(d)(\gamma,\gamma' + (1-\size{\gamma'})\dummyN ) \le d(M \uplus  O,N \uplus  O)$.
The cases where one of the \CPS{s} $M$, $N$ and $O$ are $\dummyN$ is immediate.
Hence, assume that $M$, $N$ and $O$ are not $\dummyN$.
We assume that $M=\confCPS {E_1}  {P_1}$ and $O=\confCPS {E_2}  {P_2}$, for some environments $E_1$ and $E_2$ and processes $P_1$ and $P_2$.
We proceed by case analysis on how $M \uplus O \trans{\alpha} \gamma$ is derived.
The cases are the following:
\begin{itemize}
\item
$M \uplus O \trans{\tau} \gamma$ is derived by rule \rulename{SensRead} in \autoref{tab:lts_systems_P}, instantiated as
\[
\Txiombis
{P_1 \parallel P_2 \trans{\rcva s z} P'  \Q\Q \invariantfun{}(E_1\uplus E_2) \Q\Q
\mbox{\small{$\mathit{read\_sensor}(E_1\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$}} 
}
{\confCPS{E_1 \uplus E_2} {P_1 \parallel P_2} \trans{\tau} \gamma}
\]
with $\gamma = \confCPS {\dirac{{E_1\uplus E_2}}} { \sum_{i \in I}p_i \cdot \dirac{P' \subst{v_i}{z}}}$. 
%
\item
$M \uplus  O \trans{\tau} \gamma$ is derived by rule \rulename{ActWrite} in \autoref{tab:lts_systems_P}.
%
\item
$M \uplus O \trans{\tau} \gamma$ is derived by rule \rulename{Tau} in \autoref{tab:lts_systems_P}, instantiated as
\[
\Txiombis{P_1 \parallel P_2 \trans{\tau} P' \Q\Q \invariantfun{}(E_1 \uplus E_2)}
{ \confCPS{E_1 \uplus E_2} {P_1 \parallel P_2}\trans{\tau} \gamma }
\]
with $\gamma = \confCPS {\dirac{E_1 \uplus E_2}}  {\dirac{P'}}$. 
%
%\item
%The transition $P_1 \parallel P_2 \trans{\tau} P'$ is derived by rule \rulename{Par} in \autoref{tab:lts_processes} from $P_1 \trans \tau P_1'$, where $P'_1$ is the process such that $P'=P_1'\parallel P_2$. 
%
\item
The transition $M \uplus O \trans{\tick} \gamma$ is derived by rule \rulename{Time} in \autoref{tab:lts_systems_P}, instantiated as 
 \[  \Txiombis
  {P_1\parallel P_2  \trans{\tick} {P'} \Q\Q
 \confCPS{E_1 \uplus E_2} {P_1 \parallel P_2} \ntrans{\tau} \Q\Q
\invariantfun{}(E_1 \uplus E_2)}
{\confCPS{E_1 \uplus E_2} {P_1 \parallel P_2}  \trans{\tick} \gamma}
\]
with $\gamma=\confCPS {\operatorname{next}(E)}{\dirac{P'}}$.  
%
\item
The transition $M \uplus O \trans{\inp c v} \gamma$ is derived by rule \rulename{Inp} in \autoref{tab:lts_systems_P}, instantiated as
\[
\Txiombis
{P_1 \parallel P_2 \trans{\inp c v}  P' \Q \invariantfun{}(E_1 \uplus E_2)}
{\confCPS{E_1 \uplus E_2} {P_1 \parallel P_2}  \trans{\inp c v} \gamma}
\]
with $\gamma=\confCPS {\dirac{E_1 \uplus E_2}} {\dirac{P'}}$.
%
\item
The transition $M \uplus O \trans{\out c v} \gamma$ is derived by rule \rulename{Out} in \autoref{tab:lts_systems_P}. 
\end{itemize}



We show only the first case, the other are analogous.
We recall that, by definition of operator $\uplus$, the environments $E_1$ and $E_2$ have different physical devices. 
Thus, there are two cases:
\begin{itemize}
\item 
$s$ is a sensor of $E_1$.
In this case, the transition $P_1 \parallel P_2 \trans{\rcva s z} P'$ derives by rule \rulename{Par} in \autoref{tab:lts_processes} from 
$P_1 \trans{\rcva s z} P'_1$, where $P'_1$ is a process such that $P'=P'_1 \parallel P_2$.
Moreover, the distribution $\gamma$ can be written also as $\gamma = \gamma'' \uplus \confCPS{(\dirac{E_2}}{P_2)} = \gamma'' \uplus O$, for the distribution $\gamma''$ defined as $\gamma''=\confCPS {\dirac{E_1}}  {\sum_{i \in I}p_i \cdot \dirac{P_1'\subst{v_i}{z}}}$.  

First we argue that rule \rulename{SensRead} can be used to derive a transition by $M$.
From $\invariantfun{}(E_1\uplus E_2)= \true$, by \autoref{lem:aux2P}(\ref{unobisP}) we get both $\invariantfun{}(E_1) =\true$ and $\invariantfun{}(E_2) =\true$.
From $\mathit{read\_sensor}(E_1\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$, by \autoref{lem:aux2P}(\ref{quattro})
we derive $\mathit{read\_sensor}(E_1,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$. 
Summarizing, we have $P_1 \trans{\rcva s z} P'_1$,  $\invariantfun{}(E_1)=\true$, and $\mathit{read\_sensor}(E_1,s) = \sum_{i \in I} p_i \cdot \dirac{v_i}$, which allows us to apply rule \rulename{SensRead} and derive $\confCPS{E_1}{P_1} \trans{\tau} \gamma''$, namely $M \trans{\tau} \gamma''$. 

Then, from $M \trans{\tau} \gamma''$ and $\metric (M,N) < 1$, there is a distribution $\gamma'''$ such that $N \Trans{\widehat{\tau}} \gamma'''$ with $\Kantorovich(\metric)(\gamma'',\gamma''' + (1-\size{\gamma'''})\dummyN) \le \metric(M,N)$.
Since $\invariantfun{}(E_2 )=\true $, by \autoref{lem:aux1Pbis} it follows that $N \uplus O \TransS[\widehat{\tau}]  \gamma''' \uplus O$.
Finally, we conclude that  $\gamma''' \uplus O$ is the distribution $\gamma'$ we were looking for by $\Kantorovich(d)(\gamma,\gamma''' \uplus O + (1-\size{\gamma''' \uplus O})\dummyN) = \Kantorovich(d)(\gamma'' \uplus O ,\gamma''' \uplus O + (1-\size{\gamma''' \uplus O})\dummyN) =  \Kantorovich(\metric)(\gamma'',\gamma''' (1-\size{\gamma'''})\dummyN) \le \metric(M,N) = d(M \uplus O , N \uplus O)$.
%
\item 
$s$ is a sensor of $E_2$.
In this case, the transition $P_1 \parallel P_2 \trans{\rcva s z} P'$ derives by rule \rulename{Par} in \autoref{tab:lts_processes} from 
$P_2 \trans{\rcva s z} P'_2$, where $P'_2$ is a process such that $P' =P_1 \parallel P'_2$. 
Moreover, the distribution $\gamma$ can be written also as $\gamma = \confCPS{\dirac{E_1}}{P_1} \uplus  \gamma'' = M \uplus \gamma''$, for the distribution $\gamma''$ defined as $\gamma''=\confCPS {\dirac{E_2}}  {\sum_{i \in I}p_i \cdot \dirac{P_2 '\subst{v_i}{z}}}$.  

We show that rule \rulename{SensRead} allow us to infer $N \uplus O \trans{\tau} N \uplus \gamma''$.
Assume $N = \confCPS{E_3}{P_3}$ for some environment $E_3$ and process $P_3$.
By the rule \rulename{Par} we get $P_3 \parallel P_2 \trans{\rcva s z} P_3 \parallel P'_2$.
From $\invariantfun{}(E_1\uplus E_2)= \true$, by \autoref{lem:aux2P}(\ref{unobisP}) we get both $\invariantfun{}(E_1) =\true$ and $\invariantfun{}(E_2) =\true$.
From $\metric(M ,N) < 1$ and $\invariantfun{}(E_1) =\true$,  by \autoref{lem:bis-invP} it follows that $\invariantfun{}(E_3) =\true$.
Then, $\invariantfun{}(E_3) =\true$ and $\invariantfun{}(E_2) =\true$ give, by \autoref{lem:aux2P}(\ref{quattro}), $\invariantfun{}(E_3 \uplus E_2) =\true$.
By \autoref{lem:aux2P}(\ref{quattro}), from $\mathit{read\_sensor}(E_1\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$
we derive $\mathit{read\_sensor}(E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$ and from $\mathit{read\_sensor}(E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$ we derive $\mathit{read\_sensor}(E_3\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$.
Summarising we have $P_3 \parallel P_2 \trans{\rcva s z} P_3 \parallel P'_2$, $\invariantfun{}(E_3 \uplus E_2) =\true$ and $\mathit{read\_sensor}(E_3\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$.
Hence, we can apply rule
\rulename{SensRead} to infer $N \uplus O \trans{\tau} N \uplus \gamma''$.
Finally, we can conclude that  $N \uplus \gamma''$ is the distribution $\gamma'$ we were looking for by $\Kantorovich(d)(M \uplus \gamma'',N \uplus \gamma'') = \Kantorovich(\metric)(\dirac{M},\dirac{N}) = \metric(M,N) = d(M \uplus O, N \uplus O)$.
\end{itemize}

\end{proof}



%%%%%%%%%
%%%%%%%%% PROVA DETTAGLIATA DEI VARI CASI TAGLIATA
%%%%%%%%%


\begin{comment}



%
%
\begin{itemize}
\item 
$M \uplus O \trans{\tau} \gamma$ is derived by rule \rulename{SensRead} in \autoref{tab:lts_systems_P}, instantiated as
\[
\Txiombis
{P_1 \parallel P_2 \trans{\rcva s x} P'  \Q\Q \invariantfun{}(E_1\uplus E_2) \Q\Q
\mbox{\small{$\mathit{read\_sensor}(E_1\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$}} 
}
{\confCPS{E_1 \uplus E_2} {P_1 \parallel P_2} \trans{\tau} \gamma}
\]
with $\gamma = \confCPS {\dirac{{E_1\uplus E_2}}} { \sum_{i \in I}p_i \cdot \dirac{P' \subst{v_i}{x}}}$. 
We recall that, by definition of operator $\uplus$, the environments $E_1$ and $E_2$ have different physical devices. 
Thus, there are two cases:
\begin{itemize}
\item 
$s$ is a sensor of $E_1$.
In this case, the transition $P_1 \parallel P_2 \trans{\rcva s x} P'$ derives by rule \rulename{Par} in \autoref{tab:lts_processes} from 
$P_1 \trans{\rcva s x} P'_1$, where $P'_1$ is a process such that $P'=P'_1 \parallel P_2$.
Moreover, the distribution $\gamma$ can be written also as $\gamma = \gamma'' \uplus \confCPS{(\dirac{E_2}}{P_2)} = \gamma'' \uplus O$, for the distribution $\gamma''$ defined as $\gamma''=\confCPS {\dirac{E_1}}  {\sum_{i \in I}p_i \cdot \dirac{P_1'\subst{v_i}{x}}}$.  

First we argue that rule \rulename{SensRead} can be used to derive a transition by $M$.
From $\invariantfun{}(E_1\uplus E_2)= \true$, by \autoref{lem:aux2P}(\ref{unobisP}) we get both $\invariantfun{}(E_1) =\true$ and $\invariantfun{}(E_2) =\true$.
From $\mathit{read\_sensor}(E_1\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$, by \autoref{lem:aux2P}(\ref{quattro})
we derive $\mathit{read\_sensor}(E_1,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$. 
Summarizing, we have $P_1 \trans{\rcva s x} P'_1$,  $\invariantfun{}(E_1)=\true$, and $\mathit{read\_sensor}(E_1,s) = \sum_{i \in I} p_i \cdot \dirac{v_i}$, which allows us to apply rule \rulename{SensRead} and derive $\confCPS{E_1}{P_1} \trans{\tau} \gamma''$, namely $M \trans{\tau} \gamma''$. 

Then, from $M \trans{\tau} \gamma''$ and $\metric (M,N) < 1$, there is a distribution $\gamma'''$ such that $N \Trans{\widehat{\tau}} \gamma'''$ with $\Kantorovich(\metric)(\gamma'',\gamma''' + (1-\size{\gamma'''})\dummyN) \le \metric(M,N)$.
Since $\invariantfun{}(E_2 )=\true $, by \autoref{lem:aux1Pbis} it follows that $N \uplus O \TransS[\widehat{\tau}]  \gamma''' \uplus O$.
Finally, we conclude that  $\gamma''' \uplus O$ is the distribution $\gamma'$ we were looking for by $\Kantorovich(d)(\gamma,\gamma''' \uplus O + (1-\size{\gamma''' \uplus O})\dummyN) = \Kantorovich(d)(\gamma'' \uplus O ,\gamma''' \uplus O + (1-\size{\gamma''' \uplus O})\dummyN) =  \Kantorovich(\metric)(\gamma'',\gamma''' (1-\size{\gamma'''})\dummyN) \le \metric(M,N) = d(M \uplus O , N \uplus O)$.
%
\item 
$s$ is a sensor of $E_2$.
In this case, the transition $P_1 \parallel P_2 \trans{\rcva s x} P'$ derives by rule \rulename{Par} in \autoref{tab:lts_processes} from 
$P_2 \trans{\rcva s x} P'_2$, where $P'_2$ is a process such that $P' =P_1 \parallel P'_2$. 
Moreover, the distribution $\gamma$ can be written also as $\gamma = (\dirac{E_1},P_1)  \uplus  \gamma'' = M \uplus \gamma''$, for the distribution $\gamma''$ defined as $\gamma''=\confCPS {\dirac{E_2}}  {\sum_{i \in I}p_i \cdot \dirac{P_2 '\subst{v_i}{x}}}$.  

We show that rule \rulename{SensRead} allow us to infer $N \uplus O \trans{\tau} N \uplus \gamma''$.
Assume $N = \confCPS{E_3}{P_3}$ for some environment $E_3$ and process $P_3$.
By the rule \rulename{Par} we get $P_3 \parallel P_2 \trans{\rcva s x} P_3 \parallel P'_2$.
From $\invariantfun{}(E_1\uplus E_2)= \true$, by \autoref{lem:aux2P}(\ref{unobisP}) we get both $\invariantfun{}(E_1) =\true$ and $\invariantfun{}(E_2) =\true$.
From $\metric(M ,N) < 1$ and $\invariantfun{}(E_1) =\true$,  by \autoref{lem:bis-invP} it follows that $\invariantfun{}(E_3) =\true$.
Then, $\invariantfun{}(E_3) =\true$ and $\invariantfun{}(E_2) =\true$ give, by \autoref{lem:aux2P}(\ref{quattro}), $\invariantfun{}(E_3 \uplus E_2) =\true$.
By \autoref{lem:aux2P}(\ref{quattro}), from $\mathit{read\_sensor}(E_1\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$
we derive $\mathit{read\_sensor}(E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$ and from $\mathit{read\_sensor}(E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$ we derive $\mathit{read\_sensor}(E_3\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$.
Summarising we have $P_3 \parallel P_2 \trans{\rcva s x} P_3 \parallel P'_2$, $\invariantfun{}(E_3 \uplus E_2) =\true$ and $\mathit{read\_sensor}(E_3\uplus E_2,s) = \sum_{i \in I}p_i \cdot \dirac{v_i}$.
Hence, we can apply rule
\rulename{SensRead} to infer $N \uplus O \trans{\tau} N \uplus \gamma''$.
Finally, we can conclude that  $N \uplus \gamma''$ is the distribution $\gamma'$ we were looking for by $\Kantorovich(d)(M \uplus \gamma'',N \uplus \gamma'') = \Kantorovich(\metric)(\dirac{M},\dirac{N}) = \metric(M,N) = d(M \uplus O, N \uplus O)$.
\end{itemize}
%
%
\item 
$M \uplus  O \trans{\tau} \gamma$ is derived by rule \rulename{ActWrite} in \autoref{tab:lts_systems_P}.
This case is similar to the previous one. 
Basically we apply  \autoref{lem:aux2P}(\ref{due}) instead of \autoref{lem:aux2P}(\ref{uno}),
and  \autoref{lem:aux2P}(\ref{duebis}) instead of \autoref{lem:aux2P}(\ref{unobisP}).
%
%
\item 
$M \uplus O \trans{\tau} \gamma$ is derived by rule \rulename{Tau} in \autoref{tab:lts_systems_P}, instantiated as
\[
\Txiombis{P_1 \parallel P_2 \trans{\tau} P' \Q\Q \invariantfun{}(E_1 \uplus E_2)}
{ \confCPS{E_1 \uplus E_2} {P_1 \parallel P_2}\trans{\tau} \gamma }
\]
with $\gamma = \confCPS {\dirac{E_1 \uplus E_2}}  {\dirac{P'}}$. We  can distinguish four cases.
%
\begin{itemize}
\item 
The transition $P_1 \parallel P_2 \trans{\tau} P'$ is derived by rule \rulename{Par} in \autoref{tab:lts_processes} from $P_1 \trans \tau P_1'$, where $P'_1$ is the process such that $P'=P_1'\parallel P_2$. 
Let $\gamma''$ denote the distribution $\confCPS {\dirac{E_1}}  {\dirac{P_1'}}$.  
We have that $\gamma = \gamma'' \uplus O$.

First we argue that rule \rulename{Tau} allows us to infer a transition by $M$.
Since $\invariantfun{}(E_1 \uplus E_2)$ is true, by \autoref{lem:aux2P}(\ref{quattro}) we infer that both 
$\invariantfun{}(E_1 )$ and $\invariantfun{}(E_2)$ are true. 
Since $P_1 \trans \tau P_1'$ and $\invariantfun{}(E_1 ) =\true$, we can apply rule \rulename{Tau} in \autoref{tab:lts_systems_P} to derive $M \trans{\tau} \gamma''$. 

From $M \trans{\tau} \gamma''$ and $\metric(M, N) < 1$ we infer that there is a distribution  $\gamma'''$ such that $N \TransS[\widehat{\tau}]  \gamma'''$ with $\Kantorovich(\metric)(\gamma'',\gamma''' + (1-\size{\gamma'''})\dummyN) \le \metric(M,N)$.
Since $\invariantfun{}(E_2 )=\true $, by \autoref{lem:aux1Pbis} we have that $N \TransS[\widehat{\tau}]  \gamma'''$ implies
$N \uplus O  \TransS[\widehat{\tau}]  \gamma''' \uplus O$.

Finally, we conclude that  $\gamma''' \uplus O$ is the distribution $\gamma'$ we were looking for.
In fact, we have
$\Kantorovich(d)(\gamma,\gamma''' \uplus O + (1-\size{\gamma''' \uplus O})\dummyN) = \Kantorovich(d)(\gamma'' \uplus O,\gamma''' \uplus O + (1-\size{\gamma''' \uplus O})\dummyN) = \Kantorovich(\metric)(\gamma'',\gamma''' + (1-\size{\gamma'''})\dummyN) \le \metric(M,N) = d(M \uplus O , N \uplus O)$.
 %
\item  
The transition $P_1 \parallel P_2 \trans{\tau} P'$ is derived by rule \rulename{Par}  in \autoref{tab:lts_processes}  from $P_2 \trans\tau P_2'$, where $P'_2$ is the process such that $P'=P_1\parallel P_2'$.
Let $\gamma''$ denote the distribution $\confCPS {\dirac{E_2}}  {\dirac{P_2'}}$.
We have that $\gamma = M \uplus \gamma''$.

We argue that $N \uplus O \trans{\tau}  N \uplus \gamma''$. 
Assume that $N =\confCPS {E_3}  {P_3}$, for some environment $E_3$ and process $P_3$. 
From $P_2 \trans\tau P_2'$, by rule \rulename{Par} we derive $P_3 \parallel P_2 \trans{\tau} P_3 \parallel P_2'$. 
From $\invariantfun{}(E_1\uplus E_2) = \true$, by \autoref{lem:aux2P}(\ref{quattro}) we derive both $\invariantfun{}(E_1) = \true$ and $\invariantfun{}(E_2) =\true$. 
Then, from $\invariantfun{}(E_1) = \true$ and $\metric(M,N) < 1$, by \autoref{lem:bis-invP} it follows that also
 $\invariantfun{}(E_3) =\true$.
Finally, from $\invariantfun{}(E_3) =\true$ and $\invariantfun{}(E_2) =\true$, by  \autoref{lem:aux2P}(\ref{quattro}) we get  $\invariantfun{}(E_3 \uplus E_2) =\true$.
Summarizing, we can apply rule \rulename{Tau} in \autoref{tab:lts_systems_P} with premises $P_3 \parallel P_2 \trans{\tau} P_3 \parallel P_2'$ and $\invariantfun{}(E_3 \uplus E_2) =\true$ to infer $N \uplus O \trans{\tau}  N \uplus \gamma''$. 

Finally, we can conclude that  $N \uplus \gamma'$ is the distribution $\gamma'$ we were looking for by 
$\Kantorovich(d)(\gamma, N \uplus \gamma'') = \Kantorovich(d)(M \uplus \gamma'', N \uplus \gamma'') = \Kantorovich(\metric)(\dirac{M},\dirac{N}) = \metric(M,N) = d(M \uplus O , N \uplus O)$.
%
\item 
The transition  $P_1 \parallel P_2 \trans{\tau} P'$ is derived by rule \rulename{Com}  in \autoref{tab:lts_processes} from $P_1 \trans {\out c v} P_1'$ and $P_2 \trans{\inp c v} P_2'$, where $P'_1$ and $P'_2$ are processes such that $P'=P_1'\parallel P_2'$.
We have that $\gamma = \gamma_1 \uplus \gamma_2$, where $\gamma_1 = \confCPS{\dirac{E_1}}{\dirac{P'_1}}$ and $\gamma_2 = \confCPS{\dirac{E_2}}{\dirac{P'_2}}$.

Since $\invariantfun{}( E_1 \uplus E_2) =\true$, by \autoref{lem:aux2P}(\ref{quattro}) we infer both $\invariantfun{}(E_1 )=\true$ and $\invariantfun{}(E_2) =\true$.
Since $P_1 \trans {\out c v} P_1'$ and $\invariantfun{}(E_1 ) =\true$, by rule \rulename{Out} in \autoref{tab:lts_systems_P}  we infer $\confCPS{E_1}{P_1} \trans{\out c v} \gamma_1$, namely $M \trans{\out c v} \gamma_1$. 

From $M \trans{\out c v} \gamma_1$ and $\metric(M,N) < 1$ we infer that there is a transition $N \TransS[\widehat{{\out c v}}] \gamma'_1$ with $\Kantorovich(\metric)(\gamma_1,\gamma'_1+(1-\size{\gamma'_1})\dummyN) \le \metric(M,N)$, where $N \TransS[\widehat{\out c v}] \gamma'_1$ comes from
$N \TransS[\widehat{\tau}] \gamma'' \transS[\out c v] \gamma''' \TransS[\widehat{\tau}]   \gamma'_1$ for suitable distributions $\gamma''$ and $\gamma'''$.

From $N \TransS[\widehat{\tau}] \gamma''$ and $\invariantfun{}(E_2 )=\true$, by \autoref{lem:aux1Pbis} we derive $N \uplus O \TransS[\widehat{\tau}] \gamma'' \uplus O$. 
The distribution $\gamma''$ has the form $\gamma'' = \sum_{i \in I}p_i \cdot \dirac{N_i}$ for suitable probability values $p_i$ and \CPS{s} $N_i$.
The transition $\gamma'' \TransS[\out c v] \gamma'''$ derives from $N_j \transS[\out c v] \gamma'''_j$ for all $j \in J$ and $N_i \ntransS[\out c v]$ for all $i \in I \setminus J$, for a suitable subset $J \subseteq I$ such that $\gamma''' = \sum_{j \in J} p_j \cdot \gamma'''_j$.
Consider any $j \in J$.
We observe that the \CPS{} $N_j$ has the form $N_j = \confCPS {E_1}  {P_j''}$ for a suitable process $P''_j$ such that $P''_j \transS[\out c v] P'''_j$ and $\gamma'''_j = \confCPS {\dirac{E_1}}  {\dirac{P_j'''}}$.
Since $P_2 \trans{\inp c v} P_2'$
we can use rule \rulename{Com} in \autoref{tab:lts_processes} to derive $P_j'' \parallel P_2 \trans{\tau} P_j''' \parallel P_2$.
Moreover from the fact that both $\invariantfun{}(E_1) =\true$ and  $\invariantfun{}(E_1) =\true$  
we can derive, by \autoref{lem:aux2P}(\ref{quattro}), that $\invariantfun{}(E_1 \uplus E_2) =\true$.
Summarizing, we can apply rule \rulename{Tau} in \autoref{tab:lts_systems_P} to infer $\confCPS{E_1 \uplus E_2}{P_j'' \parallel P_2} \trans{\tau} \confCPS{\dirac{E_1 \uplus E_2}}{\dirac{P_j''' \parallel P_2}}$, which gives
${\gamma''} \uplus {O}  \trans{\widehat{\tau}} {\gamma'''} \uplus {\confCPS{\dirac{E_2}}{\dirac{P'_2}}}$.
Finally, $\gamma''' \TransS[\widehat{\tau}]   \gamma'_1$ gives $\gamma''' \uplus \confCPS{\dirac{E_2}}{\dirac{P'_2}} \TransS[\widehat{\tau}]   \gamma'_1 \uplus \confCPS{\dirac{E_2}}{\dirac{P'_2}}$ by \autoref{lem:aux1Pbis}.
Henceforth we have proved  $N \uplus O \TransS[\widehat{\tau}] \gamma'' \uplus O   \trans{\tau} {\gamma'''} \uplus {\confCPS{\dirac{E_2}}{\dirac{P'_2}}}   \TransS[\widehat{\tau}]   \gamma'_1 \uplus \confCPS{\dirac{E_2}}{\dirac{P'_2}}$, namely 
$N \uplus O \TransS[\widehat{\tau}]   \gamma'_1 \uplus \confCPS{\dirac{E_2}}{\dirac{P'_2}} = \gamma'_1 \uplus \gamma_2$.

Finally, we can conclude that  $\gamma'_1 \uplus \gamma_2$ is the distribution $\gamma'$ we were looking for by 
$\Kantorovich(d)(\gamma,\gamma'_1 \uplus \gamma_2 + (1-\size{\gamma'_1 \uplus \gamma_2})\dummyN)$ = 
$\Kantorovich(d)(\gamma_1 \uplus \gamma_2,\gamma'_1 \uplus \gamma_2 + (1-\size{\gamma'_1 \uplus\gamma_2})\dummyN)$ =
$\Kantorovich(\metric)(\gamma_1, \gamma'_1 + (1-\size{\gamma'_1})\dummyN) \le \metric(M,N) = d(M \uplus O, N \uplus O)$.
%
\item 
The transition $P_1 \parallel P_2 \trans{\tau} P'$ is derived by rule \rulename{Com} in \autoref{tab:lts_processes}  from $P_1 \trans {\inp c v} P_1'$ and $P_2 \trans{\out c v} P_2'$, where $P'_1$ and $P'_2$ are processes such that $P'=P_1'\parallel P_2'$.
This case   is similar to the previous one.
\end{itemize}
%
%
\remarkR{aaggiungere caso  $\tau-\dummyN$}

\item 
The transiton $M \uplus O \trans{\tick} \gamma$ is derived by rule \rulename{Time} in \autoref{tab:lts_systems_P}, instantiated as 
 \[  \Txiombis
  {P_1\parallel P_2  \trans{\tick} {P'} \Q\Q
 \confCPS{E_1 \uplus E_2} {P_1 \parallel P_2} \ntrans{\tau} \Q\Q
\invariantfun{}(E_1 \uplus E_2)}
{\confCPS{E_1 \uplus E_2} {P_1 \parallel P_2}  \trans{\tick} \gamma}
\]
with $\gamma=\confCPS {\operatorname{next}(E)}{\dirac{P'}}$.  
As a first step, we show that rule \rulename{Time} can be used to infer transitions by both $M$ and $O$.
The transition $P_1\parallel P_2  \trans{\tick} {P'} $ is derived by rule \rulename{TimePar} in \autoref{tab:lts_processes}  from $P_1 \trans{\tick} {P'_1}$ and 
$P_2  \trans{\tick} {P'_2}$, where $P'_1$ and $P'_2$ are the processes such that $P'=P_1'\parallel P_2'$. 
From $\confCPS{E_1 \uplus E_2} {P_1 \parallel P_2} \ntrans{\tau}$, namely from $M \uplus O\ntrans{\tau}$, by \autoref{lem:aux1P} it follows that both $M \ntrans{\tau} $ and $ O \ntrans{\tau}$.
Then, since $\invariantfun{}(E_1 \uplus E_2)$ is true, by \autoref{lem:aux2P}(\ref{quattro}) we infer that both $\invariantfun{}(E_1)$ and $\invariantfun{}(E_2)$ are true. 
Summarising, we can apply rule \rulename{Time} in \autoref{tab:lts_systems_P} with premises $P_1 \trans{\tick} P'_1$, $M  \ntrans{\tau} $ and  $\invariantfun{}(E_2) = \true$ to derive
$M \trans{\tick} \confCPS{\operatorname{next}(E_1)}{\dirac{P'_1}}$.
Similarly, by the same rule, applied with premises $P_2  \trans{\tick} {P'_2} $,  $O  \ntrans{\tau}$ and $\invariantfun{}(E_2) =\true$, we derive $O \trans{\tick} \confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}}$. 
Let $\gamma_1$ and $\gamma_2$  denote the distributions $\gamma_1 = \confCPS{\operatorname{next}(E_1)}{\dirac{P'_1}}$ and $\gamma_2 = \confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}}$, respectively.

Now we observe that $\metric(M,N) < 1$ allows us to infer that the transition $M \trans{\tick} \gamma_1$ can be mimicked by a transition
$N \TransS[\widehat{\tick}] \gamma'_1$, for a distribution $\gamma'_1$ satisfying $\Kantorovich(\metric)(\gamma_1,\gamma'_1+(1-\size{\gamma'_1})\dummyN) \le \metric(M,N)$. 
The transition $N \TransS[\widehat{\tick}] \gamma'_1$ comes from
$N \TransS[\widehat{\tau}] \gamma'' \transS[\tick] \gamma''' \TransS[\widehat{\tau}]   \gamma'_1$,
for suitable distributions $\gamma''$ and $\gamma'''$.
We show that these three steps can be performed also by $N \uplus O$ to reach the configuration $\gamma'$ we are looking for, namely $N \uplus O \TransS[\widehat{\tau}] \transS[\widehat{\tick}]  \TransS[\widehat{\tau}] \gamma'$.
\begin{enumerate}
\item
First, from $N \TransS[\widehat{\tau}] \gamma''$ and $\invariantfun{}(E_2 )=\true$, by \autoref{lem:aux1Pbis} we derive $N \uplus O \TransS[\widehat{\tau}] \gamma'' \uplus O$. 
\item
Then we show that $\gamma'' \uplus O \transS[\tick]$. 
The distribution $\gamma''$ has the form $\gamma'' =\sum_{i \in I}p_i \cdot \dirac{N_i}$ for suitable probability values $p_i$ and \CPS{s} $N_i$.
The transition $\gamma'' \transS[\tick] \gamma'''$ derives from $N_j \transS[\tick] \gamma'''_j$ for all $j \in J$ and $N_i \ntransS[\tick]$ for all $i \in I \setminus J$, for a suitable subset $J \subseteq I$ such that $\gamma''' = \sum_{j \in J} p_j \cdot \gamma'''_j$.
Consider any $j \in J$.
We observe that the transition $N_j \transS[\tick] \gamma'''_j$ can be derived only by rule \rulename{Time}. 
Therefore, the premises of \rulename{Time} hold, namely the \CPS{} $N_j$ has the form $N_j = \confCPS {E_j}  {P_j''}$ for an environment $E_j$ and a process $P''_j$ such that
we have $N_j \ntransS[\tau]$,  $\invariantfun{}(E_j) =\true$ and $P''_j \transS[\tick] P'''_j$ for some process $P'''_j$.
Moreover, the process $P'''_j$ is such that $\gamma'''_j = \confCPS {\operatorname{next}(E_j)}  {\dirac{P_j'''}}$. 
%
Let $J' \subseteq J$ be the set of indexes such that, for any $j \in J'$, it holds that $N_j \uplus O  \ntrans{\tau}$. 
Consider any $j \in J'$.
We argue that by rule $\rulename{Time}$ we can infer $N_j \uplus O \transS[\tick]$.
Since $P_2 \trans{\tick} P_2'$
we can use rules \rulename{TimePar} in  \autoref{tab:lts_processes}  to derive $P_j'' \parallel P_2 \trans{\tick} P_j''' \parallel P'_2$.
Moreover, from $\invariantfun{}(E_j) =\true$ and $\invariantfun{}(E_2) =\true$
we can derive, by \autoref{lem:aux2P}(\ref{quattro}), that $\invariantfun{}(E_j \uplus E_2) =\true$.
Finally, we know that $j \in J'$ ensures $N_j \uplus O  \ntrans{\tau}$.
Therefore we can apply rule \rulename{Time} in \autoref{tab:lts_systems_P} to derive $\confCPS{E_j \uplus E_2}{P_j'' \parallel P_2} \trans{\tick} \confCPS{\operatorname{next}(E_j \uplus E_2)}{\dirac{P_j''' \parallel P'_2}} = \confCPS{\operatorname{next}(E_j)  \uplus \operatorname{next}(E_2)}{\dirac{P_j''' \parallel P'_2}}$.  
Define 
 $\widehat {\gamma'''}  = \sum_{j \in J'} p_j \cdot \gamma'''_j$. 
We derive that 
$ \gamma''   \uplus {O}  \transS[\widehat{\tick}] \widehat{\gamma'''} \uplus \confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}}$. 
\item
By $\gamma''' \TransS[\widehat{\tau}] \gamma'_1$ we immediately derive $\widehat{\gamma'''} \TransS[\widehat{\tau}]   \widehat{\gamma'_1}$.
By \autoref{lem:aux1Pbis} we have that 
$\widehat{\gamma'''} \TransS[\widehat{\tau}]   \widehat{\gamma'_1}$ implies $\widehat{\gamma'''}  \uplus (\confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}}) \TransS[\widehat{\tau}]  \widehat{\gamma'_1} \uplus (\confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}})$.
Henceforth we have proved  
$N \uplus O \TransS[\widehat{\tau}] \gamma'' \uplus O   \transS[\tick] \widehat{\gamma'''} \uplus (\confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}})  \TransS[\widehat{\tau}]  \widehat{\gamma'_1} \uplus (\confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}})$, namely 
$N \uplus O \TransS[\widehat{\tick}]   \widehat{\gamma'_1} \uplus (\confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}})$.
\end{enumerate}
To conclude that $\widehat{\gamma'_1} \uplus (\confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}})$ is the distribution $\gamma'$ we were looking for, we 
need to show that $\metric(M,N_j)=1$ for all $j \in J \setminus J'$.
In fact, this implies that 
$\Kantorovich(\metric)(\gamma_1, \widehat{\gamma'_1} + (1-\size{\widehat{\gamma'_1}})\dummyN) = \Kantorovich(\metric)(\gamma_1, \gamma'_1 + (1-\size{\gamma'_1})\dummyN)$, thus allowing us to infer
$\Kantorovich(d)(\gamma,\widehat{\gamma'_1} \uplus (\confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}}) + (1-\size{\widehat{\gamma'_1} \uplus (\confCPS{\operatorname{next}(E_2)}{P'_2}}))\dummyN)$ = 
$\Kantorovich(d)(\gamma_1 \uplus \confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}},\widehat{\gamma'_1} \uplus (\confCPS{\operatorname{next}(E_2)}{P'_2})+ (1-\size{\widehat{\gamma'_1} \uplus \confCPS{\operatorname{next}(E_2)}{\dirac{P'_2}}})\dummyN)$ = $\Kantorovich(\metric)(\gamma_1, \widehat{\gamma'_1} + (1-\size{\widehat{\gamma'_1}})\dummyN)$ =
$\Kantorovich(\metric)(\gamma_1, \gamma'_1 + (1-\size{\gamma'_1})\dummyN) \le \metric(M,N) = d(M \uplus O, N \uplus O)$.

So, let us consider any $j \in J \setminus J'$ and prove that $\metric(M,N_j)=1$.
First we note that $N_j \transS[\tick]$ implies $N_j \ntrans{\tau}$ and we remind that $O \ntrans{\tau}$.
Therefore, any transition $N_j \uplus O \transS[\tau]$ can be derived only by rule \rulename{Com} in \autoref{tab:lts_processes} and, then, rule \rulename{Tau} in \autoref{tab:lts_systems_P}.
In detail, by  \rulename{Com} we infer $P''_j \parallel P_2 \transS[\tau] P'''_j \parallel P'_2$ from either
$P''_j \transS[\overline{c} v] P'''_j$ and $P_2 \transS[cv] P'_2$ or $P''_j \transS[c v] P'''_j$ and $P_2 \transS[\overline{c}v] P'_2$, for suitable processes $P'''_j$ and $P'_2$.
Then, by \rulename{Tau} we infer $N_j \uplus O \transS[\tau]\confCPS{ \dirac{E_j \uplus E_2 }}{\dirac{P'''_j \parallel P_2}}$.
We consider the case $P''_j \transS[\overline{c} v] P'''_j$ and $P_2 \transS[cv] P'_2$, the symmetric case is analogous.
By contradiction, assume $\metric (M,N_j  )  <1$.
By rule \rulename{Out} in \autoref{tab:lts_systems_P} we infer $N_j \transS[\overline{c}v] \confCPS{\dirac{E_j}}{\dirac{P'''_j}}$ from $P''_j \transS[\overline{c} v] P'''_j$.
Then, $\metric (M,N_j  )  <1$ implies $M \TransS[\overline{c}v] \gamma$ for some distribution $\gamma$ with $\Kantorovich(\metric)(\confCPS{\dirac{E_j} }{\dirac{P'''_j}},\gamma) \le \metric(M,N)$.
This implies that $P_1 \TransS[\overline{c} v] $.
By rule \rulename{Par} we infer $P_1 \parallel P_2 \TransS[\overline{c} v]$ and, then, by rule \rulename{Tau} we derive $M \uplus O \TransS[\widehat{\tau}]\transS[\tau]$, thus contradicting 
$M \uplus O \ntransS[\tau]$.
%
\item
The transition $M \uplus O \trans{\inp c v} \gamma$ is derived by rule \rulename{Inp} in \autoref{tab:lts_systems_P}, instantiated as
\[
\Txiombis
{P_1 \parallel P_2 \trans{\inp c v}  P' \Q \invariantfun{}(E_1 \uplus E_2)}
{\confCPS{E_1 \uplus E_2} {P_1 \parallel P_2}  \trans{\inp c v} \gamma}
\]
with $\gamma=\confCPS {\dirac{E_1 \uplus E_2}} {\dirac{P'}}$. We distinguish two cases. 
\begin{itemize}
\item 
The transition $P_1 \parallel P_2 \trans{\inp c v}  P'$ is derived by rule \rulename{Par} in \autoref{tab:lts_processes} from
$P_1 \trans{\inp c v} P_1'$, where $P_1'$ is the process such that $P=P_1' \parallel P_2$.
Let $\gamma'$ denote the distribution $\gamma'=\confCPS {\dirac{E_1}}  {\dirac{P_1'}}$.
The distribution $\gamma$ can be rewritten as $\gamma = \gamma' \uplus O$.

First we show that rule \rulename{Inp} can be used to derive $M \trans{\inp c v} \gamma'$.
Since $\invariantfun{}(E_1 \uplus E_2)$ is true, by \autoref{lem:aux2P}(\ref{quattro}) we infer that 
 both $\invariantfun{}(E_1)$ and $\invariantfun{}(E_2)$ hold.
Since $P_1 \trans{\inp c v} P_1'$ and $\invariantfun{}(E_1 )=\true $, by rule \rulename{Inp} we can derive $M \trans{\inp c v} \gamma'$. 


From $M \trans{\inp c v} \gamma'$ and $\metric(M, N) < 1$, there is distribution $\gamma''$ such that $N \TransS[\widehat{\inp c v}] \gamma'' $ with $\Kantorovich(\metric)(\gamma',\gamma'' + (1-\size{\gamma''}) \dummyN) \le \metric(M,N)$.
Since $\invariantfun{}(E_2 ) =\true$, by \autoref{lem:aux1Pbis} we infer $N \uplus O \TransS[\widehat{\inp c v}]  \gamma''\uplus O$.

Finally, we can conclude that  $\gamma''\uplus O$ is the distribution $\gamma'$ we were looking for by 
$\Kantorovich(d)(\gamma,\gamma''\uplus O + (1-\size{\gamma''\uplus O})\dummyN)= \Kantorovich(d)(\gamma' \uplus O,\gamma''\uplus O + (1-\size{\gamma''\uplus O})\dummyN) = \Kantorovich(\metric)(\gamma',\gamma'' + (1-\size{\gamma''})\dummyN) \le \metric(M,N) = d(M \uplus O , N \uplus O)$.
%
\item 
The transition $P_1 \parallel P_2 \trans{\inp c v}  P'$ is derived by rule \rulename{Par} in \autoref{tab:lts_processes}  from
$P_2 \trans{\inp c v} P_2'$, where $P_2'$ is the process such that $P=P_1  \parallel P_2'$.
Let $O'=\confCPS {E_2}  {P_2'}$;  we have that  $\gamma = \dirac{M}  \uplus O'$.


Since $\invariantfun{}(E_1 \uplus E_2 ) =\true$,  by \autoref{lem:aux2P}(\ref{quattro}) it follows  that  $\invariantfun{}(E_2 )=\true $. 
Assume that $N =\confCPS {E_3}  {P_3}$, for some environemnt $E_3$ and process $P_3$.
Since $\metric(M, N) < 1$ and $\invariantfun{}(E_2 )=\true$, 
by \autoref{lem:bis-invP} we derive  $\invariantfun{}(E_3)=\true $. 
By \autoref{lem:aux2P}(\ref{quattro}) it follows that 
that  $\invariantfun{}(  E_3 \uplus E_2) =\true$.
Furthermore,  by an application of rule \rulename{Par} in  \autoref{tab:lts_processes}
 we have  $P_3 \parallel P_2 \trans{\inp c v} P_3 \parallel P_2'$.
Summarising we have
$P_3 \parallel P_2 \trans{\inp c v} P_3 \parallel P_2'$ and 
 $\invariantfun{}(E_3 \uplus E_2) =\true$.
Thus, we can apply rule \rulename{Inp} in \autoref{tab:lts_systems_P} to derive $N \uplus O \trans{\inp c v} \dirac{N} \uplus O'$. 

Finally, we can conclude that $N \uplus O'$ is the distribution we were looking for by
$\Kantorovich(d)(\gamma,\dirac{N} \uplus O') = \Kantorovich(d)(\dirac{M} \uplus O',\dirac{N} \uplus O') = \Kantorovich(\metric)(\dirac{M},{N}) = \metric(M,N) = d(M \uplus O, N \uplus O)$.
%
\end{itemize}
\item
The transition $M \uplus O \trans{\out c v} \gamma$ is derived by rule \rulename{Out} in \autoref{tab:lts_systems_P}. 
This case is similar to the previous one. 
\end{itemize}
\end{proof}

\end{comment}


%%%%%%%%%
%%%%%%%%% FINE PROVA DETTAGLIATA DEI VARI CASI TAGLIATA
%%%%%%%%%




\begin{proposition}
\label{lem:cong1Pk}
$\metric^n(M \uplus O ,N \uplus O) \le \metric^n(M , N) $, for any  physically disjoint \CPS{} $O$ and $n \ge 0$. 
\end{proposition}
\begin{proof}
We proceed by induction over $n$. 
The base case $n=0$ is immediate since $\metric^n(M,N) = \zeroF(M,N) = 0$ for all $M,N \in \nome$.
We consider the inductive step $n+1$.
The case $\metric^{n+1}(M , N) = 1$ is immediate, therefore we assume $\metric^{n+1}(M , N) < 1$. 
We have to show that any transition $M \uplus  O \trans{\alpha} \gamma$ is simulated by some transition $N \uplus  O \TransS[\widehat{\alpha}] \gamma'$ with $\Kantorovich(\metric^n)(\gamma,\gamma' + (1-\size{\gamma'})\dummyN ) \le \metric^{n+1}(M \uplus  O,N \uplus  O)$.
This can be shown precisely as in the proof of \autoref{lem:cong1P}. 
Essentially, we have to replace all occurrences of $\metric(M,N)$ by $\metric^{n+1}(M,N)$ and all occurrences of $\Kantorovich(d)(\gamma,\gamma')$ and $\Kantorovich(\metric)(\gamma,\gamma')$ by $\Kantorovich(\metric^n)(\gamma,\gamma')$.
\end{proof}

Now we prove the our weak bisimilarity metrics are preserved by parallel composition of pure-logical processes. 
These are special cases of \autoref{lem:cong1P} and \autoref{lem:cong1Pk}. 
\begin{proposition}
\label{lem:cong2P}
$\metric(M \parallel P , N \parallel P) \le \metric(M,N)$, for any pure-logical process $P$.
\end{proposition}
\begin{proof}
Let $E_\emptyset$ be the environment with an empty set of state variables, sensors and actuators. We have
$
\metric(M \parallel P , N \parallel P) \le 
\metric(M \parallel P , M \uplus (\confCPS {E_\emptyset}  {P })) + \metric(M \uplus (\confCPS {E_\emptyset}  {P }) , N \parallel P) = 
\metric(M \uplus (\confCPS {E_\emptyset}  {P }) , N \parallel P) \le
\metric(M \uplus (\confCPS {E_\emptyset}  {P }),  N \uplus (\confCPS {E_\emptyset}  {P })) + \metric(N \uplus (\confCPS {E_\emptyset}  {P }) , N \parallel P)
= \metric(M \uplus (\confCPS {E_\emptyset}  {P }) ,  N \uplus (\confCPS {E_\emptyset}  {P }))  
\le \metric(M,N)
$
where the first two inequalities follow by the triangular properties of $\metric$, the last inequality follows by \autoref{lem:cong1P} and the two equalities are immediate.
\end{proof}

\begin{proposition}
\label{lem:cong2Pk}
$\metric^n(M \parallel P , N \parallel P) \le \metric^n(M,N)$, for any pure-logical process $P$ and $n \ge 0$.
\end{proposition}
\begin{proof}
The same arguments used in the proof of \autoref{lem:cong2P} apply. 
Essentially, we simply exploits \autoref{lem:cong1Pk} instead of \autoref{lem:cong1P}.
\end{proof}



Finally, we prove that weak bisimilarity metrics are preserved by channel restriction. 
\begin{proposition}
\label{lem:cong3P}
$\metric(M {\setminus} c  , N {\setminus} c) \le \metric(M,N)$, for any channel $c$.
\end{proposition}
\begin{proof}
We reason as in \autoref{lem:cong1P}.
The case $\metric(M , N) = 1$ is immediate, therefore we assume $\metric(M , N) < 1$. 
Let us define the function $d \colon \nome \times \nome \to [0,1]$ by $d(M{\setminus} c  , N{\setminus} c ) = \metric(M,N)$ for all $M,N,O \in \nome$.
To prove the thesis it is enough to show that $d$ is a weak bisimulation metric. 
In fact, since $\metric$ is the minimal weak bisimulation metric, this implies $\metric \sqsubseteq d$, thus giving $\metric(M {\setminus} c  , N {\setminus} c ) \le d(M {\setminus} c  , N {\setminus} c ) = \metric(M,N)$.
To prove that $d$ is a weak bisimulation metric, we show that any transition $M {\setminus} c  \trans{\alpha} \gamma$ is simulated by some transition $N {\setminus} c  \TransS[\widehat{\alpha}] \gamma'$ with $\Kantorovich(d)(\gamma,\gamma' + (1-\size{\gamma'})\dummyN ) \le d(M \setminus c,N \setminus c)$.
The proof proceeds by case analysis on why $M\setminus c \trans{\alpha} \gamma$. 
\end{proof}

\begin{proposition}
\label{lem:cong3Pk}
$\metric^n(M {\setminus} c  , N {\setminus} c) \le \metric^n(M,N)$, for any channel $c$ and $n \ge 0$.
\end{proposition}
\begin{proof}
We reason as in \autoref{lem:cong1Pk}.
Hence, we proceed by induction over $n$, where the base case $n=0$ is immediate and we consider the inductive step $n+1$.
The case $\metric^{n+1}(M , N) = 1$ is immediate, therefore we assume $\metric^{n+1}(M , N) < 1$. 
We have to show that any transition $M {\setminus} c  \trans{\alpha} \gamma$ is simulated by some transition $N {\setminus} c  \TransS[\widehat{\alpha}] \gamma'$ with $\Kantorovich(\metric^n)(\gamma,\gamma' + (1-\size{\gamma'})\dummyN ) \le \metric^{n+1}(M \setminus c,N \setminus c )$.
The proof proceeds by case analysis on why $M\setminus c \trans{\alpha} \gamma$. 
\end{proof}


\noindent
\textbf{Proof of \autoref{thm:congruenceP}} \hspace{0.2 cm}
By  \autoref{lem:cong1P}--\ref{lem:cong3Pk}.
%By \autoref{lem:cong1P}, \autoref{lem:cong1Pk}, \autoref{lem:cong2P}, \autoref{lem:cong2Pk}, \autoref{lem:cong3P} and \autoref{lem:cong3Pk}.
\qed




\subsection{Proofs of  \autoref{sec:casebis}}



 

\noindent
\textbf{Proof of \autoref{prop:case-propbis}} \hspace{0.2 cm}
The proof is analogous to that of \autoref{prop:case-prop} and \autoref{prop:air3}(\ref{prop:air3.1}).
\qed
\\
%%%%%
%%%%% PROVA TAGLIATA PER ACCORCIARE IL PAPER
%%%%%

\begin{comment}
Define the \CPS{} $\mathit{NIL}$ as $\mathit{NIL}=\confCPS{E_\emptyset}{\nil}$, where $E_\emptyset$ is the empty environment.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tick} \dirac{\mathit{NIL}}$.
By \autoref{prop:sys}, \autoref{prop:X} and the fact that all evolution maps in the support of $\evolmap{}( \statefun^i{}, \actuatorfun^i{}, \uncertaintyfun{})$ are in the set of the nondeterministic version of $\evolmap{}( \statefun^i{}, \actuatorfun^i{}, \uncertaintyfun{})$ defined in \autoref{sec:case-study}, we infer that $\metric^n(\mathit{Eng_g},\mathit{NIL})=0$. 
Therefore, by the triangular property of $\metric^n$, to show the thesis $\metric^n(\mathit{Eng_g}, \widetilde{\mathit{Eng_g}})  =0$ we can show  
$\metric^n(\mathit{NIL}, \widetilde{\mathit{Eng_g}} )=0$.


The proof obligation $\metric^n(\mathit{NIL}, \widetilde{\mathit{Eng_g}} )\leq   0$ follows from the following five properties, by observing that the system $\widetilde{\mathit{Eng_g}}$ satisfies the first one.
\remarkS{Ancora puntini}
\begin{enumerate}
\item  
\label{prop:case-prop1b}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) =0$ 
whenever the state of the environment $E$ satisfies $\mathit{cool} = \off$ and $\mathit{temp} \in [0, 11.5 ]$, and the process $P$ is $\mathit{Ctrl}$, or $\tick.\mathit{Ctrl}$, or $\mathit{Cooling}$. 
%
\item   
\label{prop:case-prop2b}
$\metric^n(\mathit{NIL},\confCPS{E}{P })=0$ 
whenever  the state of the environment $E$ satisfies $\mathit{cool} = \on$ and $\mathit{temp} \in (9.9, 11.5 ]$, and the process $P$ is 
\[ 
P =\fix Y \tick^5 .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.Y}
{\wact{\off}{\mathit{cool}}.\tick. \mathit{Ctrl}} .
\]
%
\item   
\label{prop:case-prop3b}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) =0$,  
for all $n \in [1,4]$,
whenever  the state of the environment $E$
satisfies $\mathit{cool}=\on$ and $\mathit{temp} \in  (9.9 -k(1.2),11.5 -k (0.4) ]$ and the process $P$ is
\[ 
P =\tick^{5-k} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } .
\]
%
\item   
\label{prop:case-prop5b}
$\metric^n(\mathit{NIL},\confCPS{E}{P })=0$ 
whenever the state of the environment $E$
satisfies  $\mathit{cool}=\on$ and $\mathit{temp}  \le  9.9$ and the process $P$ is
\[ 
P =   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}} .
\]
% 
\item   
\label{prop:case-prop6b}
$\metric^n(\mathit{NIL},\confCPS{E}{P}) =0$ 
whenever the state of the environment $E$
satisfies $\mathit{cool}= \on$ and $\mathit{temp}  \le  9.9$ and the process $P$ is
$P = {\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}}$.
\end{enumerate}

We prove these five properties in parallel, by induction over $n$.
The base case $n=0$ is immediate since $\metric^0$ is the constant zero function $\zeroF$.
We consider the inductive step $n > 0$.
First we observe that, given any distribution $\sum_{i \in I} p_i \cdot \dirac{M_i}$ over $\CPS{s}$, the only matching $\omega \in \Omega(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})$ is  $\omega(M_i,\mathit{NIL})= p_i$. 
It follows that $\Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})=
 \sum_{i \in I} p_i  \metric^{n-1}(M_i,\mathit{NIL})$.
\begin{enumerate}
\item  
We distinguish the cases $P=\mathit{Ctrl}$, $P=\tick.\mathit{Ctrl}$ and $P=\mathit{Cooling}$.
\begin{itemize}
\item
Case $P=\mathit{Ctrl}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tau}  \sum_{i \in I} p_i \cdot \dirac{M_i}$, 
where $M_i= \confCPS{E}{P_i }$, with either $P_i=\tick.\mathit{Ctrl}$ or  $P_i=\mathit{Cooling}$.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})$.
By the inductive hypothesis on \autoref{prop:case-prop1b} we infer
$\metric^{n-1}(M_i,\mathit{NIL})  =0$
in both cases, thus implying
\[
  \Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})=\sum_{i \in I} p_i  \metric^{n-1}(M_i,\mathit{NIL})=0 .
\]
which completes the proof.
%
\item
Case $P=\tick.\mathit{Ctrl}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{\mathit{Ctrl}}}$.
Again, the only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{\mathit{Ctrl}}},\dirac{\mathit{NIL}})$.
Notice that in all environments $E'$ in the support of  $\mathit{next}(E)$ we have $\mathit{cool} = \off$.
Therefore  $\mathit{temp} \le 10.1$ in $E$ and $\mathit{temp} \in [0, 10.1+1.4 ]= [0,  11.5 ]$ in $E'$, thus implying that we can apply the inductive hypothesis on \autoref{prop:case-prop1b} to get
$\metric^{n-1} (\confCPS{E'}{\mathit{Ctrl}},\mathit{NIL})  =0$.
It follows
\[
 \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{\mathit{Ctrl}}} ,\dirac {\mathit{NIL}}) \le  1-\left( 1- q_g (p_g)^5  \right)^{n-1} =0
\]
which completes the proof.
%
\item
Case $P=\mathit{Cooling}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P}  \trans{\tau} \dirac{M}$ with
\[
M= \confCPS{E'}{\fix Y \tick^5 .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.Y}
{\wact{\off}{\mathit{cool}}.\tick. \mathit{Ctrl}} }.
 \] 
Again, the only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\dirac{M},\dirac{\mathit{NIL}})$.
Notice that in the environment of $M$ we have $\mathit{cool} = \on$ and, since the system detected a temperature $\mathit{temp} > 10$, we are sure that the effective value of the temperature was $\mathit{temp} \in [9.9, 11.5 ]$, thus implying that we can apply the inductive hypothesis on \autoref{prop:case-prop2b}  to get
$\metric^{n-1} (M,\mathit{NIL}) =0$.
It follows
\[
   \Kantorovich(\metric^{n-1})( \dirac{M},\dirac {\mathit{NIL}})=  \metric^{n-1} (M,\mathit{NIL}) \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} 
   \le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which completes the proof.
\end{itemize}
%
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{P'}}$ with
\[ 
P' =\tick^{4} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } .
\]
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{P'}},\dirac{\mathit{NIL}})$.
By definition, 
$\mathit{next}(E)=  \sum_{v \in [0.4,1.2]_g}  \frac{1}{|[0.4,1.2]_g|} \overline{E [\mathit{temp} \mapsto \statefun{}(temp) - v]}$
Hence in all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ lies   in the interval $(9.9 - k(1.2),11.5-k(0.4))]$ with $n=1$. 
We can apply  the inductive hypothesis on \autoref{prop:case-prop3b} to get
$\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL}) =0$.
Therefore  we have
\[
  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})
= 0 
\]
which completes the proof.
%
\item  
%$M= \confCPS{E'}{P }  $ dove  il $\mathit{cool}$ e' $\on$ e la   $\mathit{temp} \in  (11.4 -k(0.3),11.5 -k (0.3) ] $ in $E'$, e, \[ P =\tick^{5-k} .   \rsens x {s_{\operatorname{t}}}  \ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}} {\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } \] $k \in [1,4]$
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E')}{ \dirac{P'}}$ with
 \[ 
P' =\tick^{5-k-1} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } 
\]
We distinguish two cases, namely $n \in [1,3]$ and $n=4$.
Let us start with $n \in [1,3]$.
In all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ lies   in the interval $(9.9- (k+1)(1.2),11.5-(k+1)(0.4))]$.
We can apply  the inductive hypothesis on \autoref{prop:case-prop3b} to get
$
\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})  =0
$ 
Therefore  we have
\[
  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})=0\]
Consider now the case $k=4$.
%We have
%$
%P'=\rsens x {s_{\operatorname{t}}}  
%\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
%{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} }$
In all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ lies   in the interval $(9.9- (k+1)(1.2),11.5-(k+1)(0.4))]=(3.3,9.5]$.

We can apply  the inductive hypothesis on \autoref{prop:case-prop5b} to get
$ \metric^{n-1} (\confCPS{E''}{ P'} )=0$.
Therefore we have
\[
   \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})
=0 \]
which completes the proof.
%

\item   
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tau}   \confCPS{\dirac{E}}{\dirac{P'}}$, with
$P'= \wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}$.
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\dirac{E}}{\dirac{P'}},\dirac{\mathit{NIL}})$.
Since the environment $E$ satisfies $\mathit{cool}=\on$ and $\mathit{temp}  \le  9.9$,
we can apply the inductive hypothesis on \autoref{prop:case-prop6b}
to get
 $ \metric^{n-1} (\confCPS{E}{P'}  ,\mathit{NIL})  =0 $.
It follows
\[
  \Kantorovich(\metric^{n-1})(\confCPS{\dirac{E}}{\dirac{P'}},\dirac {\mathit{NIL}})=  \metric^{n-1} (\confCPS{E}{P'},\mathit{NIL})=0
\]
which completes the proof.
%  
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P}  \trans{\tau}  \confCPS{\dirac{\operatorname{update\_act}(E,\mathit{cool},\mathit{off})}}{\dirac{\tick.\mathit{Ctrl} }}$.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\dirac{\operatorname{update\_act}(E,\mathit{cool},\mathit{off})}}{\dirac{\tick.\mathit{Ctrl} }}{\dirac{P'}},\dirac{\mathit{NIL}})$ 
=  
$\metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}),\mathit{NIL})$.
Since the environment $\operatorname{update\_act}(E,\mathit{cool},\mathit{off})$ differs with respect to $E$ only in the value of $\mathit{cool}$, we have $\mathit{cool} = \off$ and $\mathit{temp} \le 9.9$, and we can apply the inductive hypothesis on \autoref{prop:case-prop1b} to get
$ \metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}) ,\mathit{NIL})  = 0 $.
It follows
\[
\metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}),\mathit{NIL})=0
\]
which completes the proof.
\end{enumerate}
\end{proof}

\end{comment}
%%%%%
%%%%% END PROVA TAGLIATA PER ACCORCIARE IL PAPER
%%%%%

\begin{comment}
\noindent 
\textbf{Proof of \autoref{prop:air2}}
\begin{proof}
By \autoref{prop:case-propbis} we derive 
$\metric^n (\mathit{Eng }_g, \widehat{\mathit{Eng }_g}) =0$, for any $n \in \mathbb{N}$.
Hence, we have that
\[
 \metric  (\mathit{Eng }_g, \widehat{\mathit{Eng }_g}) =
\lim_{n\rightarrow \infty}\metric^n (\mathit{Eng }_g, \widehat{\mathit{Eng }_g}) =0.
\]
By simple 
$\alpha$-conversion it follows that 
$\metric (\mathit{Eng }_g^{\mathrm L} , \widehat{\mathit{Eng }_g^{\mathrm L}}) =
\metric (\mathit{Eng }_g^{\mathrm R} , \widehat{\mathit{Eng }_g^{\mathrm R}}) =0$. 
By \autoref{thm:congruenceP}(1) (and transitivity) it 
follows that 
$
\metric (\mathit{Eng}_g^{\mathrm L} \uplus \mathit{Eng}_g^{\mathrm R},
\widetilde{\mathit{Eng}_g^{\mathrm L}} \uplus \widetilde{\mathit{Eng}_g^{\mathrm R}}) =0$.
By \autoref{thm:congruenceP}(2) it follows that 
\[
\metric \left(
 \left(  \mathit{Eng}_g^{\mathrm{L}}  
\uplus 
(   \mathit{Eng}_g^{\mathrm R}  \right) \parallel \mathit{Check},
 \left( \widehat{\mathit{Eng}_g^{\mathrm{L}} } 
\uplus 
(  \widehat{\mathit{Eng}_g^{\mathrm R}} \right) \parallel \mathit{Check}
\right)=0.
 \]
By \autoref{thm:congruence}(3) we
obtain  $\metric \left(  \mathit{Airplane}_g  , \widetilde{\mathit{Airplane}_g} \right)=0  $ and hence
$  \mathit{Airplane}_g  \approx_0  \widetilde{\mathit{Airplane}_g} $.

\end{proof}
\end{comment}




%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% PROVA CON ESPONENTE 5 ANZICHE' 6 TAGLIATA 
%%%%%%%%%%%%%%%%

\begin{comment}
\noindent
\textbf{Proof of \autoref{prop:case-prop}} 
We start by showing that 
$\frac{\mid [0.3, 0.4)_g \mid}{\mid [0.3, 1.1]_g \mid} =  \frac{1 }{8+ 10^{-g+1}} $.
We have that $  \mid [0.3, 1.1]_{g} \mid = (1.1-0.3) 10^{g}+1 = 8 \left( 10^{g-1}\right) +1$ and, since $0.4 \not \in [0.3, 0.4)$, 
we have that 
$\mid [0.3, 0.4)_{g} \mid= (0.4-0.3) 10^{ g} = 10^{g -1} $.
Hence we conclude that
$\frac{10^{g-1}}{8 \left(10^{g -1}\right) +1}  =  \frac{1 }{8+ 10^{-g+1}}$.

Define the \CPS{} $\mathit{NIL}$ as $\mathit{NIL}=\confCPS{E_\emptyset}{\nil}$, where $E_\emptyset$ is the empty environment.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tick} \dirac{\mathit{NIL}}$.
By \autoref{prop:sys}, \autoref{prop:X} and the fact that all evolution maps in the support of $\evolmap{}( \statefun^i{}, \actuatorfun^i{}, \uncertaintyfun{})$ are in the set of the nondeterministic version of $\evolmap{}( \statefun^i{}, \actuatorfun^i{}, \uncertaintyfun{})$ defined in \autoref{sec:case-study}, we infer that $\metric^n(\mathit{Eng_g},\mathit{NIL})=0$. 
Therefore, by the triangular property of $\metric^n$, to show the thesis $\metric^n(\mathit{Eng_g}, \widehat{\mathit{Eng_g}}) \le  1- \left(1- (p_g)^5\right)^n$ we can show  
$\metric^n(\mathit{NIL}, \widehat{\mathit{Eng_g}} )\leq   1- \left(1- (p_g)^5\right)^n$.

The proof obligation $\metric^n(\mathit{NIL}, \widehat{\mathit{Eng_g}} )\leq   1- \left(1- (p_g)^5\right)^n$ follows from the following six properties, by observing that the system $\widehat{\mathit{Eng_g}}$ satisfies the first one.
\remarkS{Scrivere una frase per i puntini}
\remarkR{Ho dato un nome a rec y}
In the following we denote the process $\fix{Y} \tick^5 .   \rsens x {s_{\operatorname{t}}} . \ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.Y}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} }$ with $\mathit{RecY}$. 
\begin{enumerate}
\item  
\label{prop:case-prop1}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le 1-\left( 1- q_g (p_g)^5  \right)^n$ 
whenever the state of the environment $E$ satisfies $\mathit{cool} = \off$ and $\mathit{temp} \in [0, 11.5 ]$, and the process $P$ is $\mathit{Ctrl}$, or $\tick.\mathit{Ctrl}$, or $\mathit{Cooling}$. 
%
\item   
\label{prop:case-prop2}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le  1-\left( 1- q_g (p_g)^5  \right)^n$ 
whenever  the state of the environment $E$ satisfies $\mathit{cool} = \on$ and $\mathit{temp} \in (9.9, 11.5 ]$, and the process $P$ is 
$\mathit{RecY}$.
%
\item   
\label{prop:case-prop3}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le 1- \left( 1- (p_g)^{5-k} \right)   \left( 1- q_g (p_g)^5  \right)^n$,  
for all $n \in [1,4]$,
whenever  the state of the environment $E$
satisfies $\mathit{cool}=\on$ and $\mathit{temp} \in  (11.4 -k(0.3),11.5 -k (0.3) ]$ and the process $P$ is
\[ 
P =\tick^{5-k} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } .
\]
\item   
\label{prop:case-prop4}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le1-\left( 1- q_g (p_g)^5  \right)^n$ 
whenever the state of the environment $E$
satisfies $\mathit{cool} = \on$ and $\mathit{temp}  \le    11.4 -k (0.3)$, and the process $P$ is
 \[ P =\tick^{5-k} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}} \]
for any $k\in [1,4]$.
%
\item   
\label{prop:case-prop5}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le1-\left( 1- q_g (p_g)^5  \right)^n$ 
whenever the state of the environment $E$
satisfies  $\mathit{cool}=\on$ and $\mathit{temp}  \le  9.9$ and the process $P$ is
\[ 
P =   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}} .
\]
% 
\item   
\label{prop:case-prop6}
$\metric^n(\mathit{NIL},\confCPS{E}{P}) \le  1-\left( 1- q_g (p_g)^5  \right)^n$ 
whenever the state of the environment $E$
satisfies $\mathit{cool}= \on$ and $\mathit{temp}  \le  9.9$ and the process $P$ is
$P = {\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}}$.
\end{enumerate}

We prove these six properties in parallel, by induction over $n$.
The base case $n=0$ is immediate since $\metric^0$ is the contant zero function $\zeroF$.
We consider the inductive step $n > 0$.
First we observe that, given any distribution $\sum_{i \in I} p_i \cdot \dirac{M_i}$ over $\CPS{s}$, the only matching $\omega \in \Omega(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})$ is  $\omega(M_i,\mathit{NIL})= p_i$. 
It follows that $\Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})=
 \sum_{i \in I} p_i  \metric^{n-1}(M_i,\mathit{NIL})$.
We give the proof of the third case, which is the most interesting one.
The others are similar.

The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E')}{ \dirac{P'}}$ with
 \[ 
P' =\tick^{5-k-1} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } 
\]
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tick} \dirac{\mathit{NIL}}$.
We infer $\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})( \confCPS{\mathit{next}(E')}{ \dirac{P'}},\dirac{\mathit{NIL}} )$.
We distinguish two cases, namely $k \in [1,3]$ and $k=4$.
Let us start with $k \in [1,3]$.
In all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ lies either in the interval $(11.4 - (k+1)(0.3),11.5-(k+1)(0.3))]$, with a probability bounded by $p_g$, whereas $\mathit{temp}$ is below $11.4 - (k+1)(0.3)$ with a probability not less that $1-p_g$.
In the first case we can apply  the inductive hypothesis on \autoref{prop:case-prop3} to get
$
\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le 1- \left(1- (p_g)^{5-k-1}\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} 
$,
whereas in the second case we can apply  the inductive hypothesis on \autoref{prop:case-prop4} to get
$\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le    1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore for some $q \le p_g$ we have
%
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})\\

= &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q \left( 1- \left(1- (p_g)^{5-k-1}\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} \right)   
\\  
\le &        1   -   \left(1 -p_g (p_g)^{  5-k-1}\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -   \left(1 -  (p_g)^{5-k}\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\end{array} 
\]
and the thesis follows.

Consider now the case $k=4$.
In all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ is above $9.9$, with a probability bounded by $p_g$, and below $9.9$  with a probability not less that $1-p_g$.
In the first case we simply known that $\metric^{n-1} (\confCPS{E'}{P'}) \le 1$ by the definition of $\metric^n$, whereas in the second case we can apply  the inductive hypothesis on \autoref{prop:case-prop5} to get
$ \metric^{n-1} (\confCPS{E''}{ P'} )   \le    1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore, for some $q \le p_g$ we have
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})
\\
\le &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q    
\\  
=   &     1-\left( 1- q_g (p_g)^5  \right)^{n-1 }   - q+ q\left( 1- q_g (p_g)^5  \right)^{n-1 }    +
 q  
\\ 
=   &     1   -   \left(1 -q \right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\ 
\le &        1   -   \left(1 -p_g \right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
\end{array} 
\]
and the thesis follows also in this case.
\qed
\\


%%%%%
%%%%% CASI TAGLIATI PER ACCORCIARE IL PAPER, COMPRESO QUELLO LASCIATO
%%%%% DELLA PROVA TAGLIATA PER ESPONENTE 5
%%%%%


\begin{enumerate}
\item  
We distinguish the cases $P=\mathit{Ctrl}$, $P=\tick.\mathit{Ctrl}$ and $P=\mathit{Cooling}$.
\begin{itemize}
\item
Case $P=\mathit{Ctrl}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tau}  \sum_{i \in I} p_i \cdot \dirac{M_i}$, 
where $M_i= \confCPS{E}{P_i }$, with either $P_i=\tick.\mathit{Ctrl}$ or  $P_i=\mathit{Cooling}$.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})$.
By the inductive hypothesis on \autoref{prop:case-prop1} we infer
$\metric^{n-1}(M_i,\mathit{NIL})  \le 1- \left( 1- q_g (p_g)^5  \right)^{n-1}$
in both cases, thus implying
\[
  \Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})=\sum_{i \in I} p_i  \metric^{n-1}(M_i,\mathit{NIL})\le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}  \le 1-\left( 1- q_g (p_g)^5  \right)^{n} .
\]
which completes the proof.
%
\item
Case $P=\tick.\mathit{Ctrl}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{\mathit{Ctrl}}}$.
Again, the only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{\mathit{Ctrl}}},\dirac{\mathit{NIL}})$.
Notice that in all environments $E'$ in the support of  $\mathit{next}(E)$ we have $\mathit{cool} = \off$.
Therefore  $\mathit{temp} \le 10.1$ in $E$ and $\mathit{temp} \in [0, 10.1+1.4 ]= [0,  11.5 ]$ in $E'$, thus implying that we can apply the inductive hypothesis on \autoref{prop:case-prop1} to get
$\metric^{n-1} (\confCPS{E'}{\mathit{Ctrl}},\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
It follows
\[
 \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{\mathit{Ctrl}}} ,\dirac {\mathit{NIL}}) \le  1-\left( 1- q_g (p_g)^5  \right)^{n-1} \le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which completes the proof.
%
\item
Case $P=\mathit{Cooling}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P}  \trans{\tau} \dirac{M}$ with
\[
M= \confCPS{E'}{\mathit{RecY}}.
 \] 
Again, the only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\dirac{M},\dirac{\mathit{NIL}})$.
Notice that in the environment of $M$ we have $\mathit{cool} = \on$ and, since the system detected a temperature $\mathit{temp} > 10$, we are sure that the effective value of the temperature was $\mathit{temp} \in [9.9, 11.5 ]$, thus implying that we can apply the inductive hypothesis on \autoref{prop:case-prop2}  to get
$\metric^{n-1} (M,\mathit{NIL}) \le  1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
It follows
\[
   \Kantorovich(\metric^{n-1})( \dirac{M},\dirac {\mathit{NIL}})=  \metric^{n-1} (M,\mathit{NIL}) \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} 
   \le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which completes the proof.
\end{itemize}
%
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{P'}}$ with
\[ 
P' =\tick^{4} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } .
\]
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{P'}},\dirac{\mathit{NIL}})$.
By definition, 
$\mathit{next}(E)=  \sum_{v \in [0.3,1.1]_g}  \frac{1}{|[0.3,1.1]_g|} \overline{E [\mathit{temp} \mapsto \statefun{}(temp) - v]}$
Hence in all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ lies   in the interval $(11.4 - k(0.3),11.5-k(0.3))]$, with $n=1$, with a probability bounded by $p_g$, whereas $\mathit{temp}$ is below $11.4 - k(0.3)$ with a probability not less that $1-p_g$.
In the first case we can apply  the inductive hypothesis on \autoref{prop:case-prop3} to get
$
\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le 1- \left(1- (p_g)^4\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} 
$,
whereas in the second case we can apply  the inductive hypothesis on \autoref{prop:case-prop4} to get
$\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le    1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore for some $q \le p_g$ we have
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})
\\
= &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q \left( 1- \left(1- (p_g)^4\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} \right)   
\\  
=   &    \left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) - q\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right)  +
 q  \left(  1- \left(1- (p_g)^4\right)   \left( 1- q_g (p_g)^5  \right)^{n-1}\right) 
\\
=   &     1-\left( 1- q_g (p_g)^5  \right)^{n-1 }   - q+ q\left( 1- q_g (p_g)^5  \right)^{n-1 }    +
 q  -  \left(q- q(p_g)^4\right)    \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1 -q+q   -   \left(1- q + q-q (p_g)^4\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -   \left(1 -q (p_g)^4\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
\le &        1   -   \left(1 -p_g (p_g)^4\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -   \left(1 -  (p_g)^5\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -      \left( 1- q_g (p_g)^5  \right)^{n  } 
\end{array} 
\]
which completes the proof.
%
\item   
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E')}{ \dirac{P'}}$ with
 \[ 
P' =\tick^{5-k-1} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } 
\]
We distinguish two cases, namely $n \in [1,3]$ and $n=4$.
Let us start with $n \in [1,3]$.
In all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ lies either in the interval $(11.4 - (k+1)(0.3),11.5-(k+1)(0.3))]$, with a probability bounded by $p_g$, whereas $\mathit{temp}$ is below $11.4 - (k+1)(0.3)$ with a probability not less that $1-p_g$.
In the first case we can apply  the inductive hypothesis on \autoref{prop:case-prop3} to get
$
\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le 1- \left(1- (p_g)^{5-k-1}\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} 
$,
whereas in the second case we can apply  the inductive hypothesis on \autoref{prop:case-prop4} to get
$\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le    1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore for some $q \le p_g$ we have
%
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})\\

= &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q \left( 1- \left(1- (p_g)^{5-k-1}\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} \right)   
\\  
\le &        1   -   \left(1 -p_g (p_g)^{  5-k-1}\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -   \left(1 -  (p_g)^{5-k}\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\end{array} 
\]
Consider now the case $n=4$.
In all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ is above $9.9$, with a probability bounded by $p_g$, and below $9.9$  with a probability not less that $1-p_g$.
In the first case we simply known that $\metric^{n-1} (\confCPS{E'}{P'}) \le 1$ by the definition of $\metric^n$, whereas in the second case we can apply  the inductive hypothesis on \autoref{prop:case-prop5} to get
$ \metric^{n-1} (\confCPS{E''}{ P'} )   \le    1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore, for some $q \le p_g$ we have
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})
\\
\le &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q    
\\  
=   &     1-\left( 1- q_g (p_g)^5  \right)^{n-1 }   - q+ q\left( 1- q_g (p_g)^5  \right)^{n-1 }    +
 q  
\\ 
=   &     1   -   \left(1 -q \right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\ 
\le &        1   -   \left(1 -p_g \right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
\end{array} 
\]
which completes the proof.
%
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{P'}}$, with
 \[ 
P' =\tick^{5-k-1} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}} 
\]
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{ \tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{P'}},\dirac{\mathit{NIL}})$.
We have 
$\mathit{next}(E)=  \sum_{v \in [0.3,1.1]_g}  \frac{1}{|[0.3,1.1]_g|} \overline{E [\mathit{temp} \mapsto  \statefun{}(temp) - v]}$, 
thus implying that for all environments $E'$ in the support of $\mathit{next}(E)$ we have
$\mathit{cool} = \on$ and
 $\mathit{temp}  \le    11.4 -(k+1) (0.3)$. 
Therefore, if $n<4$ then  in $E'$ we have $\mathit{cool} = on$ and $\mathit{temp} \le 11.4 - (k+1)0.3$, with $n+1 \in [1,4]$, so that we can apply the inductive hypothesis on \autoref{prop:case-prop4} and get 
$ \metric^{n-1} (\confCPS{E'}{P'},\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Otherwise, if $n=4$ then  in $E'$ we have $\mathit{cool} = on$ and $\mathit{temp} \le 9.9$, 
so that we can apply the inductive hypothesis on \autoref{prop:case-prop5} and get 
$ \metric^{n-1} (\confCPS{E'}{P'},\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}$
also in this case.
It follows
\[
  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E)}{ \dirac{\mathit{P'}}} ,\dirac {\mathit{NIL}})
  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} 
\le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which concludes the proof.
%
\item   
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tau}   \confCPS{\dirac{E}}{\dirac{P'}}$, with
$P'= \wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}$.
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\dirac{E}}{\dirac{P'}},\dirac{\mathit{NIL}})$.
Since the environment $E$ satisfies $\mathit{cool}=\on$ and $\mathit{temp}  \le  9.9$,
we can apply the inductive hypothesis on \autoref{prop:case-prop6}
to get
 $ \metric^{n-1} (\confCPS{E}{P'}  ,\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} $.
It follows
\[
  \Kantorovich(\metric^{n-1})(\confCPS{\dirac{E}}{\dirac{P'}},\dirac {\mathit{NIL}})=  \metric^{n-1} (\confCPS{E}{P'},\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} 
  \le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which completes the proof.
%  
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P}  \trans{\tau}  \confCPS{\dirac{\operatorname{update\_act}(E,\mathit{cool},\mathit{off})}}{\dirac{\tick.\mathit{Ctrl} }}$.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\dirac{\operatorname{update\_act}(E,\mathit{cool},\mathit{off})}}{\dirac{\tick.\mathit{Ctrl} }}{\dirac{P'}},\dirac{\mathit{NIL}})$ 
=  
$\metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}),\mathit{NIL})$.
Since the environment $\operatorname{update\_act}(E,\mathit{cool},\mathit{off})$ differs with respect to $E$ only in the value of $\mathit{cool}$, we have $\mathit{cool} = \off$ and $\mathit{temp} \le 9.9$, and we can apply the inductive hypothesis on \autoref{prop:case-prop1} to get
$ \metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}) ,\mathit{NIL})  \le  1-\left( 1- q_g (p_g)^5  \right)^{n-1} $.
It follows
\[
\metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}),\mathit{NIL})
 \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}  
 \le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which completes the proof.
\end{enumerate}
\end{proof}
\end{comment}
%%%%%
%%%%% END CASI TAGLIATI PER ACCORCIARE IL PAPER, COMPRESO QUELLO LASCIATO
%%%%% PER CASI TAGLIATI CON ESPONENTE 5
%%%%%


%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%END  PROVA CON ESPONENTE 5 ANZICHE' 6 TAGLIATA 
%%%%%%%%%%%%%%%%



 










\noindent
\textbf{Proof of \autoref{prop:case-prop}} \hspace{0.2 cm}
%We start by showing that 
%$\frac{\mid [0.3, 0.4)_g \mid}{\mid [0.3, 1.1]_g \mid} =  \frac{1 }{8+ 10^{-g+1}} $.
%We have that $  \mid [0.3, 1.1]_{g} \mid = (1.1-0.3) 10^{g}+1 = 8 \left( 10^{g-1}\right) +1$ and, since $0.4 \not \in [0.3, 0.4)$, 
%we have that 
%$\mid [0.3, 0.4)_{g} \mid= (0.4-0.3) 10^{ g} = 10^{g -1} $.
%Hence we conclude that
%$\frac{10^{g-1}}{8 \left(10^{g -1}\right) +1}  =  \frac{1 }{8+ 10^{-g+1}}$.
%In a similar way we  can  prove that 
%$q_g=\frac{\mid (1.3, 1.4]_g \mid}{\mid [0.6, 1.4]_g \mid} =  \frac{1 }{8+ 10^{-g+1}} $.
%Indeed we have that $\mid (1, 1.1]_g \mid= (10.5-10.4) 10^{ g} = 10^{g -1} $.
Define the \CPS{} $\mathit{NIL}$ as $\mathit{NIL}=\confCPS{E_\emptyset}{\nil}$, where $E_\emptyset$ is the empty environment.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tick} \dirac{\mathit{NIL}}$.
By \autoref{prop:sys} and \autoref{prop:X} 
%and the fact that all evolution maps in the support of $\evolmap{}( \statefun^i{}, \actuatorfun^i{}, \uncertaintyfun{})$ are in the set of the nondeterministic version of $\evolmap{}( \statefun^i{}, \actuatorfun^i{}, \uncertaintyfun{})$ defined in \autoref{sec:case-study}, 
we infer that $\metric^n(\mathit{Eng_g},\mathit{NIL})=0$.
 %\remarkR{nonn capisco, forse e' rimasta da una vecchia versione} 
Therefore, by the triangular property of $\metric^n$, to show the thesis $\metric^n(\mathit{Eng_g}, \widehat{\mathit{Eng_g}}) \le  1- \left(1- q_g(p_g)^5\right)^n$ we can show  
$\metric^n(\mathit{NIL}, \widehat{\mathit{Eng_g}} )\leq   1- \left(1-q_g (p_g)^5\right)^n$.

The proof obligation $\metric^n(\mathit{NIL}, \widehat{\mathit{Eng_g}} )\leq   1- \left(1- (p_g)^5\right)^n$ follows from the following nine properties, by observing that the system $\widehat{\mathit{Eng_g}}$ satisfies the first one.
In the following we denote the process $\fix{Y} \tick^5 .   \rsens x {s_{\operatorname{t}}} . \ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.Y}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} }$ with $\mathit{RecY}$. 
\begin{enumerate}
\item  
\label{prop:case-prop1a}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le 1-\left( 1-  q_g (p_g)^5 \right)^n$ 
whenever the state of the environment $E$ satisfies $\mathit{cool} = \off$ and $\mathit{temp} \in [0, 10.1] $, and the process $P$ is $\mathit{Ctrl}$, or $\tick.\mathit{Ctrl}$. 
%
\item  
\label{prop:case-prop1b}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le 1-\left( 1-    q_g(p_g)^5  \right)^n$ 
whenever the state of the environment $E$ satisfies $\mathit{cool} = \off$ and $\mathit{temp} \in (10.1, 11.4 ]$, and the process $P$ is $\mathit{Ctrl}$,   or $\mathit{Cooling}$. 
%
%
\item  
\label{prop:case-prop1c}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le 1-\left( 1-   (p_g)^5  \right)\left( 1-  q_g (p_g)^5  \right)^n$ 
whenever the state of the environment $E$ satisfies $\mathit{cool} = \off$ and $\mathit{temp} \in (10.4, 11.5 ]$, and the process $P$ is $\mathit{Ctrl}$,   or $\mathit{Cooling}$. 
%
\item   
\label{prop:case-prop2a}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le  1-\left( 1-  q_g (p_g)^5  \right)^n$ 
whenever  the state of the environment $E$ satisfies $\mathit{cool} = \on$ and $\mathit{temp} \in (9.9, 11.4 ]$, and the process $P$ is 
$\mathit{RecY}$.
%
\item   
\label{prop:case-prop2b}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le  1-\left( 1-   (p_g)^5  \right)\left( 1-  q_g (p_g)^5  \right)^n$ 
whenever  the state of the environment $E$ satisfies $\mathit{cool} = \on$ and $\mathit{temp} \in (10.4, 11.5 ]$, and the process $P$ is 
$\mathit{RecY}$.
%
\item   
\label{prop:case-prop3}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le 1- \left( 1- (p_g)^{5-k} \right)   \left( 1- q_g (p_g)^5  \right)^n$,  
for all $n \in [1,4]$,
whenever  the state of the environment $E$
satisfies $\mathit{cool}=\on$ and $\mathit{temp} \in  (11.4 -k(0.3),11.5 -k (0.3) ]$ and the process $P$ is
\[ 
P =\tick^{5-k} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } .
\]
\item   
\label{prop:case-prop4}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le1-\left( 1- q_g (p_g)^5  \right)^n$ 
whenever the state of the environment $E$
satisfies $\mathit{cool} = \on$ and $\mathit{temp}  \le    11.4 -k (0.3)$, and the process $P$ is
 \[ P =\tick^{5-k} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}} \]
for any $k\in [1,4]$.
%
\item   
\label{prop:case-prop5}
$\metric^n(\mathit{NIL},\confCPS{E}{P }) \le1-\left( 1- q_g (p_g)^5  \right)^n$ 
whenever the state of the environment $E$
satisfies  $\mathit{cool}=\on$ and $\mathit{temp}  \le  9.9$ and the process $P$ is
\[ 
P =   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}} .
\]
% 
\item   
\label{prop:case-prop6}
$\metric^n(\mathit{NIL},\confCPS{E}{P}) \le  1-\left( 1- q_g (p_g)^5  \right)^n$ 
whenever the state of the environment $E$
satisfies $\mathit{cool}= \on$ and $\mathit{temp}  \le  9.9$ and the process $P$ is
$P = {\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}}$.
\end{enumerate}

We prove these nine properties in parallel, by induction over $n$.
The base case $n=0$ is immediate since $\metric^0$ is the constant zero function $\zeroF$.
We consider the inductive step $n > 0$.
First we observe that, given any distribution $\sum_{i \in I} p_i \cdot \dirac{M_i}$ over $\CPS{s}$, the only matching $\omega \in \Omega(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})$ is  $\omega(M_i,\mathit{NIL})= p_i$. 
It follows that $\Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})=
 \sum_{i \in I} p_i  \metric^{n-1}(M_i,\mathit{NIL})$.
We show only the first property, the other are analogous.

%\begin{enumerate}
%\item  

We distinguish the cases $P=\mathit{Ctrl}$ and $P=\tick.\mathit{Ctrl}$.
\begin{itemize}
\item
Case $P=\mathit{Ctrl}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tau}  \sum_{i \in I} p_i \cdot \dirac{M_i}$, 
where $M_i= \confCPS{E}{P_i }$, with either $P_i=\tick.\mathit{Ctrl}$ or  $P_i=\mathit{Cooling}$.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})$.
By the inductive hypothesis on \autoref{prop:case-prop1a} we infer
$\metric^{n-1}(M_i,\mathit{NIL})  \le 1- \left( 1- q_g (p_g)^5  \right)^{n-1}$
in both cases, thus implying
\[
  \Kantorovich(\metric^{n-1})(\sum_{i \in I} p_i \cdot \dirac{M_i},\dirac {\mathit{NIL}})=\sum_{i \in I} p_i  \metric^{n-1}(M_i,\mathit{NIL})\le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}  \le 1-\left( 1- q_g (p_g)^5  \right)^{n} .
\]
which completes the proof.
%
\item
Case $P=\tick.\mathit{Ctrl}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{\mathit{Ctrl}}}$.
Again, the only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{\mathit{Ctrl}}},\dirac{\mathit{NIL}})$.
By definition, 
$\mathit{next}(E)=  \sum_{v \in [0.3,1.1]_g}  \frac{1}{|[0.3,1.1]_g|} \overline{E [\mathit{temp} \mapsto \statefun{}(temp) - v]}$.
Hence in all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \off$ and
the temperature $\mathit{temp}$ lies   in the interval $[0+0.3 ,10.1+1.4]$.

We have two cases: $\mathit{temp}   \in [0+0.3 ,10.1]$, and $ \mathit{temp}   \in (10.1 ,10.5]$.
If $\mathit{temp}   \in [0+0.3 ,10.1]$, then by the inductive hypothesis on \autoref{prop:case-prop1a} we infer
$\metric^{n-1}(\confCPS{ E' }{ \dirac{\mathit{Ctrl}}},\mathit{NIL})  \le 1- \left( 1- q_g (p_g)^5  \right)^{n-1}$
 thus implying
\[
  \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{\mathit{Ctrl}}},\dirac {\mathit{NIL}})
  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}  \le 1-\left( 1- q_g (p_g)^5  \right)^{n} .
\]

If $\mathit{temp}   \in (10.1 ,10.5]$, then $\mathit{temp}   \in (10.4 ,10.5]$ 
with a probability bounded by $q_g$, whereas $\mathit{temp}  \in (10.1 ,10.4] $ with a probability not less that $1-q_g$.
If $\mathit{temp}   \in (10.4 ,10.5]$  we can apply  the inductive hypothesis on \autoref{prop:case-prop1c} to get
$
\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le  1-\left( 1-  (p_g)^5  \right)\left( 1-  q_g (p_g)^5  \right)^{n-1} 
$.
If $\mathit{temp}   \in (10.4 ,10.5]$ we can apply  the inductive hypothesis on \autoref{prop:case-prop1b} to get
$\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le     1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore for some $q \le q_g$ we have
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})
\\
= &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q    \left( 1-   (p_g)^5  \right)  \left( 1-  q_g (p_g)^5  \right)^{n-1}
\\  
=   &    \left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) - q\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right)  +
 q   \left( 1-   (p_g)^5  \right) \left( 1-  q_g (p_g)^5  \right)^{n-1}
\\
=   &     1-\left( 1- q_g (p_g)^5  \right)^{n-1 }   - q+ q\left( 1- q_g (p_g)^5  \right)^{n-1 }    +
 q  -  \left(q- q(p_g)^5\right)    \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1 -q+q   -   \left(1- q + q-q (p_g)^5\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -   \left(1 -q (p_g)^5\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
\le   &     1   -   \left(1 - q_g (p_g)^5\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -      \left( 1- q_g (p_g)^5  \right)^{n  } 
\end{array} 
\]
which completes the proof.
%
\end{itemize}
\qed

%%%%%%%
%%%%%%% CASI 2-8 TAGLIATI PER SNELLIRE
%%%%%%%
%
\begin{comment}
\item  
We distinguish the cases $P=\mathit{Ctrl}$  and $P=\mathit{Cooling}$.
\begin{itemize}
\item
Case $P=\mathit{Ctrl}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tau}  \sum_{i \in I} p_i \cdot  \confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}}=
\confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}}$.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(
\confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}},\dirac {\mathit{NIL}})$.
Since   $\mathit{temp} \in (10.1,11.4 ]$, by the inductive hypothesis on \autoref{prop:case-prop1b} we infer
\[
  \Kantorovich(\metric^{n-1})(
\confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}},\dirac {\mathit{NIL}})=
 \metric^{n-1} (\confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}},\dirac {\mathit{NIL}} )
\le 1-\left( 1- q_g  (p_g)^5  \right)^{n-1}  
\le 1-\left( 1- q_g  (p_g)^5  \right)^{n} .
\]
which completes the proof.

%
\item
Case $P=\mathit{Cooling}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P}  \trans{\tau}  \confCPS{\dirac{ E'}}{\dirac{ \mathit{RecY}}}$.

Again, the only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})( \confCPS{\dirac{ E'}}{\dirac{ \mathit{RecY}}},\dirac{\mathit{NIL}})$.
Notice that in the environment   $E'$ we have $\mathit{cool} = \on$ and,  $\mathit{temp} \in (10.1,10.4 ]$,    implying that we can apply the inductive hypothesis on \autoref{prop:case-prop2a}  to get
$\metric^{n-1} (  \confCPS{\dirac{ E'}}{\dirac{ \mathit{RecY}}},\mathit{NIL}) \le  1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
It follows
\[
   \Kantorovich(\metric^{n-1})(   \confCPS{\dirac{ E'}}{\dirac{ \mathit{RecY}}},\dirac {\mathit{NIL}})=  \metric^{n-1} (  \confCPS{\dirac{ E'}}{\dirac{ \mathit{RecY}}},\mathit{NIL}) \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} 
   \le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which completes the proof.
\end{itemize}
%
\item  
We distinguish the cases $P=\mathit{Ctrl}$  and $P=\mathit{Cooling}$.
\begin{itemize}
\item
Case $P=\mathit{Ctrl}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tau}  \sum_{i \in I} p_i \cdot  \confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}}=
\confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}}$.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(
\confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}},\dirac {\mathit{NIL}})$.
Since  $\mathit{temp} \in (11.4,11.5 ]$, by the inductive hypothesis on \autoref{prop:case-prop1c} we infer

$
\begin{array}{rlr}
&
  \Kantorovich(\metric^{n-1})(
\confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}},\dirac {\mathit{NIL}})\\
=&
 \metric^{n-1} (\confCPS{\dirac{E}}{ \dirac{ \mathit{Cooling}}},\dirac {\mathit{NIL}} )\\
\le & 1-\left( 1-    (p_g)^5  \right)\left( 1-  q_g (p_g)^5  \right)^{n-1}  \\
\le & 1-\left( 1-    (p_g)^5  \right)\left( 1-  q_g (p_g)^5  \right)^n .\\
\end{array}
$

which completes the proof.
%

%
\item
Case $P=\mathit{Cooling}$.\\
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P}  \trans{\tau} \dirac{  \confCPS{E'}{\mathit{RecY}}}$.

Again, the only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\dirac{M},\dirac{\mathit{NIL}})$.
Notice that in the environment  $E'$ we have $\mathit{cool} = \on$ and,  $\mathit{temp} \in (10.4,10.5 ]$,   implying that we can apply the inductive hypothesis on \autoref{prop:case-prop2b}  to get
$\metric^{n-1} ( \dirac{  \confCPS{E'}{\mathit{RecY}}},\mathit{NIL}) \le  1-\left( 1-   (p_g)^5  \right)\left( 1-  q_g (p_g)^5  \right)^{n-1}$.
It follows

$
\begin{array}{rlr}
  &  \Kantorovich(\metric^{n-1})(  \dirac{  \confCPS{E'}{\mathit{RecY}}},\dirac {\mathit{NIL}})\\
   = & \metric^{n-1} ( \dirac{  \confCPS{E'}{\mathit{RecY}}},\mathit{NIL})\\
    \le & 1-\left( 1-  (p_g)^5  \right)\left( 1-  q_g (p_g)^5  \right) ^{n-1}\\
   \le  & 1-\left( 1-   (p_g)^5  \right)\left( 1-  q_g (p_g)^5  \right)^n\\
\end{array} 
$

which completes the proof.
\end{itemize}
%
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{P'}}$, with
 \[ 
P' =\tick^{4} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}} 
\]
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{ \tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{P'}},\dirac{\mathit{NIL}})$.
We have 
$\mathit{next}(E)=  \sum_{v \in [0.3,1.1]_g}  \frac{1}{|[0.3,1.1]_g|} \overline{E [\mathit{temp} \mapsto  \statefun{}(temp) - v]}$, 
thus implying that for all environments $E'$ in the support of $\mathit{next}(E)$ we have
$\mathit{cool} = \on$ and
 $\mathit{temp}  \le    11.4 - k (0.3)$ with $k=1$. 
Therefore,   we can apply the inductive hypothesis on \autoref{prop:case-prop4} and get 
$ \metric^{n-1} (\confCPS{E'}{P'},\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
It follows
\[
  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E)}{ \dirac{\mathit{P'}}} ,\dirac {\mathit{NIL}})
  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} 
\le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which concludes the proof.
%
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{P'}}$ with
\[ 
P' =\tick^{4} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } .
\]
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{P'}},\dirac{\mathit{NIL}})$.
By definition, 
$\mathit{next}(E)=  \sum_{v \in [0.3,1.1]_g}  \frac{1}{|[0.3,1.1]_g|} \overline{E [\mathit{temp} \mapsto \statefun{}(temp) - v]}$
Hence in all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ lies   in the interval $(11.4 - k(0.3),11.5-k(0.3))]$, with $k=1$, with a probability bounded by $p_g$, whereas $\mathit{temp}$ is below $11.4 - k(0.3)$ with a probability not less that $1-p_g$.
In the first case we can apply  the inductive hypothesis on \autoref{prop:case-prop3} to get
$
\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le 1- \left(1- (p_g)^4\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} 
$,
whereas in the second case we can apply  the inductive hypothesis on \autoref{prop:case-prop4} to get
$\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le    1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore for some $q \le p_g$ we have
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})
\\
= &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q \left( 1- \left(1- (p_g)^4\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} \right)   
\\  
=   &    \left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) - q\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right)  +
 q  \left(  1- \left(1- (p_g)^4\right)   \left( 1- q_g (p_g)^5  \right)^{n-1}\right) 
\\
=   &     1-\left( 1- q_g (p_g)^5  \right)^{n-1 }   - q+ q\left( 1- q_g (p_g)^5  \right)^{n-1 }    +
 q  -  \left(q- q(p_g)^4\right)    \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1 -q+q   -   \left(1- q + q-q (p_g)^4\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -   \left(1 -q (p_g)^4\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
\le &        1   -   \left(1 -p_g (p_g)^4\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -   \left(1 -  (p_g)^5\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -      \left( 1- q_g (p_g)^5  \right)^{n  } 
\end{array} 
\]
which completes the proof.
%
\item   
%$M= \confCPS{E'}{P }  $ dove  il $\mathit{cool}$ e' $\on$ e la   $\mathit{temp} \in  (11.4 -k(0.3),11.5 -k (0.3) ] $ in $E'$, e, \[ P =\tick^{5-k} .   \rsens x {s_{\operatorname{t}}}  \ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}} {\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } \] $k \in [1,4]$ 
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E')}{ \dirac{P'}}$ with
 \[ 
P' =\tick^{5-k-1} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} } 
\]
We distinguish two cases, namely $k \in [1,3]$ and $k=4$.
Let us start with $k \in [1,3]$.
In all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ lies either in the interval $(11.4 - (k+1)(0.3),11.5-(k+1)(0.3))]$, with a probability bounded by $p_g$, whereas $\mathit{temp}$ is below $11.4 - (k+1)(0.3)$ with a probability not less that $1-p_g$.
In the first case we can apply  the inductive hypothesis on \autoref{prop:case-prop3} to get
$
\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le 1- \left(1- (p_g)^{5-k-1}\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} 
$,
whereas in the second case we can apply  the inductive hypothesis on \autoref{prop:case-prop4} to get
$\metric^{n-1} (\confCPS{E'}{ P'},\mathit{NIL})   \le    1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore for some $q \le p_g$ we have
%
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})\\

= &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q \left( 1- \left(1- (p_g)^{5-k-1}\right)   \left( 1- q_g (p_g)^5  \right)^{n-1} \right)   
\\  
\le &        1   -   \left(1 -p_g (p_g)^{  5-k-1}\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
=   &     1   -   \left(1 -  (p_g)^{5-k}\right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\end{array} 
\]
Consider now the case $k=4$.
%We have
%$
%P'=\rsens x {s_{\operatorname{t}}}  
%\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
%{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl} }$
In all environments $E'$  in the support of $\mathit{next}(E)$ we have $\mathit{cool} = \on$ and
the temperature $\mathit{temp}$ is above $9.9$, with a probability bounded by $p_g$, and below $9.9$  with a probability not less that $1-p_g$.
In the first case we simply known that $\metric^{n-1} (\confCPS{E'}{P'}) \le 1$ by the definition of $\metric^n$, whereas in the second case we can apply  the inductive hypothesis on \autoref{prop:case-prop5} to get
$ \metric^{n-1} (\confCPS{E''}{ P'} )   \le    1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Therefore, for some $q \le p_g$ we have
\[
\begin{array}{rlr}
&  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E')}{ \dirac{P'}} ,\dirac {\mathit{NIL}})
\\
\le &   (1-q)\left(  1-\left( 1- q_g (p_g)^5  \right)^{n-1 } \right) + 
q    
\\  
=   &     1-\left( 1- q_g (p_g)^5  \right)^{n-1 }   - q+ q\left( 1- q_g (p_g)^5  \right)^{n-1 }    +
 q  
\\ 
=   &     1   -   \left(1 -q \right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\ 
\le &        1   -   \left(1 -p_g \right)      \left( 1- q_g (p_g)^5  \right)^{n-1} 
\\
\end{array} 
\]
which completes the proof.
%
%
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tick} \confCPS{\mathit{next}(E)}{ \dirac{P'}}$, with
 \[ 
P' =\tick^{5-k-1} .   \rsens x {s_{\operatorname{t}}}  
\ifelse {x>10} {\OUT{\mathit{warning}}{\mathrm{ID}}.\mathit{RecY}}
{\wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}} 
\]
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{ \tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\mathit{next}(E)}{ \dirac{P'}},\dirac{\mathit{NIL}})$.
We have 
$\mathit{next}(E)=  \sum_{v \in [0.3,1.1]_g}  \frac{1}{|[0.3,1.1]_g|} \overline{E [\mathit{temp} \mapsto  \statefun{}(temp) - v]}$, 
thus implying that for all environments $E'$ in the support of $\mathit{next}(E)$ we have
$\mathit{cool} = \on$ and
 $\mathit{temp}  \le    11.4 -(k+1) (0.3)$. 
Therefore, if $k<4$ then  in $E'$ we have $\mathit{cool} = on$ and $\mathit{temp} \le 11.4 - (k+1)0.3$, with $k+1 \in [1,4]$, so that we can apply the inductive hypothesis on \autoref{prop:case-prop4} and get 
$ \metric^{n-1} (\confCPS{E'}{P'},\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}$.
Otherwise, if $k=4$ then  in $E'$ we have $\mathit{cool} = on$ and $\mathit{temp} \le 9.9$, 
so that we can apply the inductive hypothesis on \autoref{prop:case-prop5} and get 
$ \metric^{n-1} (\confCPS{E'}{P'},\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}$
also in this case.
It follows
\[
  \Kantorovich(\metric^{n-1})(  \confCPS{\mathit{next}(E)}{ \dirac{\mathit{P'}}} ,\dirac {\mathit{NIL}})
  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} 
\le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which concludes the proof.
%

\item   
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P} \trans{\tau}   \confCPS{\dirac{E}}{\dirac{P'}}$, with
$P'= \wact{\off}{\mathit{cool}}.\tick.\mathit{Ctrl}$.
Again, the only transition by system $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore we infer that
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\dirac{E}}{\dirac{P'}},\dirac{\mathit{NIL}})$.
Since the environment $E$ satisfies $\mathit{cool}=\on$ and $\mathit{temp}  \le  9.9$,
we can apply the inductive hypothesis on \autoref{prop:case-prop6}
to get
 $ \metric^{n-1} (\confCPS{E}{P'}  ,\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} $.
It follows
\[
  \Kantorovich(\metric^{n-1})(\confCPS{\dirac{E}}{\dirac{P'}},\dirac {\mathit{NIL}})=  \metric^{n-1} (\confCPS{E}{P'},\mathit{NIL})  \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1} 
  \le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which completes the proof.
%  
\item  
The only transition by $\confCPS{E}{P}$ is 
$\confCPS{E}{P}  \trans{\tau}  \confCPS{\dirac{\operatorname{update\_act}(E,\mathit{cool},\mathit{off})}}{\dirac{\tick.\mathit{Ctrl} }}$.
The only transition by $\mathit{NIL}$ is $\mathit{NIL} \trans{\tau} \dirac{\mathit{NIL}}$.
Therefore 
$\metric^n(\confCPS{E}{P},\mathit{NIL}) \le \Kantorovich(\metric^{n-1})(\confCPS{\dirac{\operatorname{update\_act}(E,\mathit{cool},\mathit{off})}}{\dirac{\tick.\mathit{Ctrl} }}{\dirac{P'}},\dirac{\mathit{NIL}})$ 
=  
$\metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}),\mathit{NIL})$.
Since the environment $\operatorname{update\_act}(E,\mathit{cool},\mathit{off})$ differs with respect to $E$ only in the value of $\mathit{cool}$, we have $\mathit{cool} = \off$ and $\mathit{temp} \le 9.9$, and we can apply the inductive hypothesis on \autoref{prop:case-prop1a} to get
$ \metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}) ,\mathit{NIL})  \le  1-\left( 1- q_g (p_g)^5  \right)^{n-1} $.
It follows
\[
\metric^{n-1} (\operatorname{update\_act}(E,\mathit{cool},\mathit{off}),\mathit{NIL})
 \le 1-\left( 1- q_g (p_g)^5  \right)^{n-1}  
 \le 1-\left( 1- q_g (p_g)^5  \right)^{n}
\]
which completes the proof.
\end{enumerate}

\end{comment}

%%%%%%%
%%%%%%% CASI 2-8 TAGLIATI PER SNELLIRE
%%%%%%%

 


\noindent 
\textbf{Proof of \autoref{prop:air3}} \hspace{0.2 cm}
By \autoref{prop:case-prop} we derive 
$\metric^n(\mathit{Eng }_g, \widehat{\mathit{Eng }_g}) \le  1- \left(1- q_g(p_g)^5\right)^n=p$.
By simple 
$\alpha$-conversion it follows that 
$\metric^n(\mathit{Eng }_g^{\mathrm L} , \widehat{\mathit{Eng }_g^{\mathrm L}}) \le p$ and 
$\metric^n(\mathit{Eng }_g^{\mathrm R} , \widehat{\mathit{Eng }_g^{\mathrm R}}) \le  p$, respectively. 
By \autoref{thm:congruenceP}(\ref{thm:congruence1Pk}) (and transitivity) it 
follows that 
$
\metric^n(\mathit{Eng}_g^{\mathrm L} \uplus \mathit{Eng}_g^{\mathrm R},
\widetilde{\mathit{Eng}_g^{\mathrm L}} \uplus \widetilde{\mathit{Eng}_g^{\mathrm R}}) \le 2p$.
By \autoref{thm:congruenceP}(\ref{thm:congruence2Pk}) it follows that 
\[
\metric^n\left(
 \left(  \mathit{Eng}_g^{\mathrm{L}}  
\uplus 
(   \mathit{Eng}_g^{\mathrm R}  \right) \parallel \mathit{Check},
 \left( \widehat{\mathit{Eng}_g^{\mathrm{L}} } 
\uplus 
(  \widehat{\mathit{Eng}_g^{\mathrm R}} \right) \parallel \mathit{Check}
\right) \le 2p.
 \]
By \autoref{thm:congruence}(\ref{thm:congruence3Pk}) we
obtain  $\metric^n\left(  \mathit{Airplane}_g  , \widetilde{\mathit{Airplane}_g} \right) \le 2p  $.
Finally, from this fact  a by \autoref{eq:lim},  we derive
\[
\lim_{ g \rightarrow +\infty}   \metric^n( \mathit{Airplane}_g  ,  \widetilde{\mathit{Airplane}_g}  )\leq 2\left(1- \left(1- \frac{1}{8^6}  \right)^n\right).
\]
\qed

